Abatement of Ionizing Radiation for Superconducting Quantum Devices

Ionizing radiation has been shown to reduce the performance of superconducting quantum circuits. In this report, we evaluate the expected contributions of different sources of ambient radioactivity for typical superconducting qubit experiment platforms. Our assessment of radioactivity inside a typical cryostat highlights the importance of selecting appropriate materials for the experiment components nearest to qubit devices, such as packaging and electrical interconnects. We present a shallow underground facility (30-meter water equivalent) to reduce the flux of cosmic rays and a lead shielded cryostat to abate the naturally occurring radiogenic gamma-ray flux in the laboratory environment. We predict that superconducting qubit devices operated in this facility could experience a reduced rate of correlated multi-qubit errors by a factor of approximately 20 relative to the rate in a typical above-ground, unshielded facility. Finally, we outline overall design improvements that would be required to further reduce the residual ionizing radiation rate, down to the limit of current generation direct detection dark matter experiments.

==> dosetable.tex <==
\begin{table}[ht!]
    \centering
    \caption{Simulated interaction rate and dose from some components inside the dilution refrigerator. The estimated residual rates from cosmic rays in the SUL and external gammas passing through the shield are included for comparison. For coax cables and connectors, MMCX connectors and RG174 cables are used as the closest available entries in the literature. 
    }
    \label{tab:internalrate}
    \sisetup{separate-uncertainty, table-align-uncertainty=false, table-align-exponent=false}
    \begin{tabular}{|llc|S[table-format=3.1e-1]|S[table-format=2.1e-1]|}
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\toprule
        \hline
        Component & Material & {Mass} & {Interaction rate} & {Dose rate} \\
        & & {(kg)} & {($10^{-3}$~cts/s/g)} & {(keV/s/g)} \\
        \hline
        Cosmic rays in SUL &  &  & {$\sim$}30 & {$\sim$}7 \\
        \multicolumn{3}{|l|}{Ambient gammas (no shield)} & 420 & 50 \\
        \multicolumn{3}{|l|}{Ambient gammas (shielded)} & 0.8 & 0.1 \\
        \multicolumn{3}{|l|}{Gamma shield (see below)}  & 1 & 0.1 \\
        \multicolumn{3}{|l|}{All DR components (see below)} & 0.2 & 0.04 \\
        \multicolumn{3}{|l|}{All instrumentation (see below)}  & 0.5 & 0.1 \\
        %\multicolumn{2}{l}{Ceramic PCB (interposer)} & & \sim150 & \sim50 \\
        \hline
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        \hline
        \multicolumn{5}{|l|}{Ceramic PCB interposers (\emph{Not} included in above totals)} \\
        \hline
        \quad interposer & alumina & 0.001 & 36 & 13 \\
        \quad interposer & Rogers RO4350B & 0.001 & 160 & 65 \\
        \quad interposer & Rogers TMM10 & 0.001 & 250 & 92 \\
        \hline
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        \hline
        \multicolumn{5}{|l|}{Individual contributions to ``Gamma Shield''}\\
        \hline
        \quad Lead bricks (\iso{Pb}{210}) & Pb & 6200 & 0.67 & 0.050 \\
        %\quad Other isotopes in lead & Pb & 6200  & 1e-4 & 2e-5 \\
        %\quad Lower support & Al & 120 & 0.4 & 0.05 \\
        %\quad Upper support & Al & 22 & 0.02 & 2e-4 \\
        \quad Inner support & Al & 140 & 0.41 & 0.051 \\
        \hline

        %\multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\hline
        \multicolumn{5}{|l|}{Individual contributions to ``All DR components''} \\
        \hline

        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\toprule
        \hline
        Component & Material & {Mass} & {Interaction rate} & {Dose rate} \\
        & & {(kg)} & {($10^{-3}$~cts/s/g)} & {(keV/s/g)} \\
        \hline
        
        
        \quad Experiment stage & Cu/Au & 2.1 & 0.015 & 0.0022 \\
        \quad MXC stage & Cu/Au & 4.1 & 0.0032  & 4.4e-4 \\
        \quad CP stage & Cu/Au & 3.1 & 4.5e-4 & 5.9e-5 \\
        \quad Still stage & Cu/Au & 6.1 & 3.0e-4 & 4.0e-5 \\
        \quad 4K stage & Cu & 9 & 8.7e-5 & 1.2e-5\\
        \quad 50K stage & Cu & 5 & 1.6e-5 & 2.0e-6\\
        \quad Vacuum flange & steel & 20 & 7.2e-4 & 8.4e-5\\

        \quad Experiment shield & Cu/Al/mumetal & 3 & 0.11 & 0.014 \\
        \quad Still can & Cu & 6.8 & 0.0018 & 2.8e-4\\
        \quad 4K can & Al & 4.3 & 0.062 & 0.0086\\
        \quad 50K can & Al & 6 & 0.044 & 0.0065\\
        \quad Vacuum can & Al & 22 & 0.13 & 0.019 \\
        \hline

        %\multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\hline
        %\multicolumn{5}{|l|}{Individual contributions to ``All Instrumentation''} \\
        %\hline
        \quad Wirebonds & Al/Si & {$10\times\SI{0.1}{mg}$} & 0.0028 & 0.0012 \\
        \quad Interposer & TMM10 & 0.001 & & \\
        \quad Package & Cu & {\SI{100}{g}} & 0.037 & 0.010 \\
        \quad \quad Coax connectors & SMA & {$10\times\SI{2.3}{g}$} & 0.37 & 0.11 \\
        \quad \quad Fasteners & brass & {$10\times\SI{0.3}{g}$} & 0.0044 & 0.0012 \\
        \quad Closest coax cable & semirigid & {$10\times\SI{10}{cm}$} & 1.7e-4 & 2.4e-5 \\
        \quad MXC RF feedthroughs & SMA & {$20\times\SI{2.3}{g}$} & 0.0011 & 1.4e-4 \\
        %\quad MXC DC feedthroughs & BeCu & {25\times10 ct} & 0.0026 & 3.1e-4 \\
        %\quad Readout amps, etc. & resistor & {100 ct} & 1.3e-5 & 1.6e-6 \\
        \hline
        %\bottomrule
    \end{tabular}
\end{table}


==> dosetable_unshielded_surface.tex <==
\begin{table}[ht!]
    \centering
    \caption{Simulated interaction rate and dose for a silicon chip from environmental gammas, cosmic rays, and trace radioactivity inside the fridge for an unshielded system at sea level. 
    }
    \label{tab:internalrate}
    \sisetup{separate-uncertainty, table-align-uncertainty=false, table-align-exponent=false}
    \begin{tabular}{|llc|S[table-format=3.1e-1]|S[table-format=3.1e-1]|}
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\toprule
        \hline
        Component & Material & {Mass} & {Interaction rate} & {Dose rate} \\
        & & {(kg)} & {($10^{-3}$~cts/s/g)} & {(keV/s/g)} \\
        \hline
        \multicolumn{3}{|l|}{Cosmic rays (chip horizontal)} & 290 & 52 \\
        \multicolumn{3}{|l|}{Cosmic rays (chip vertical)} & 190 & 49 \\
        \multicolumn{3}{|l|}{Ambient Gammas} & 420 & 53 \\
        \multicolumn{3}{|l|}{Ceramic PCB interposers} & & \\
        \quad  & alumina & \SI{370}{mg} & 29 & 11 \\
        \quad  & RO4350B & \SI{780}{mg} & 63 & 24 \\
        \quad  & TMM10   & \SI{550}{mg} & 140 & 52 \\
        \multicolumn{3}{|l|}{Coax connectors on package} &  &  \\
        \quad inside (line-of-sight) & SMA & {$10\times\SI{2.3}{g}$} & 530 & 190\\
        \quad outside (no line-of-sight) & SMA & {$10\times\SI{2.3}{g}$} & 8.9 & 1.1 \\
        Bump bonds & indium &{\SI{20}{\mu g}} & 0.28 & 0.030 \\
        \multicolumn{3}{|l|}{All other components (itemized below)} & 0.72 & 0.11 \\
        \hline
        \multicolumn{3}{|l|}{\quad Fridge stages and shields} & 0.23 & 0.033 \\
        \quad \quad MXC stage & Cu & 4.6 & 0.0027  & 4.0e-4 \\
        \quad \quad CP stage & Cu & 3.3 & 2.9e-4 & 3.9e-5 \\
        \quad \quad Still stage & Cu & 5.9 & 2.1e-4 & 2.9e-5 \\
        \quad \quad 4K stage & Cu & 8.7 & 8.6e-5 & 1.1e-5\\
        \quad \quad 50K stage & Cu & 5.1 & 1.6e-5 & 2.0e-6\\
        \quad \quad Vacuum flange & steel & 21 & 7.9e-4 & 9.8e-5\\
        \quad \quad Still can & Cu & 6.3 & 0.0019 & 2.7e-4\\
        \quad \quad 4K can & Al & 4.1 & 0.058 & 0.0083\\
        \quad \quad 50K can & Al & 5.7 & 0.047 & 0.0070\\
        \quad \quad Vacuum can & Al & 21 & 0.11 & 0.015 \\
        \quad \quad Gold plating & gold & 0.5 & 0.010 & 0.0014\\
        \hline
        \multicolumn{3}{|l|}{\quad Experiment readout} & 0.49 & 0.074 \\
        \quad \quad Wirebonds & Al/Si & {$10\times\SI{0.1}{mg}$} & 0.0029 & 0.0012 \\
        \quad \quad Package & Cu & 0.1 & 0.042 & 0.012 \\
        \quad \quad Package Fasteners & brass & {$10\times\SI{0.3}{g}$} & 0.0045 & 0.0012 \\
        \quad \quad Cryo filters & K\&L & {$10\times\SI{15}{g}$} & 0.10 & 0.015\\
        \quad \quad Closest coax cable & semirigid & {$10\times\SI{10}{cm}$} & 4.5e-6 & 6.2e-7 \\
        \quad \quad Coldfinger & Cu & 1.8 & 0.0065 & 9.7e-4 \\
        \quad \quad Inner shield &  &  & 0.11 & 0.014 \\
        & Cu & 1 & 9.9e-4 & 1.5e-4\\
        & Al & 1 & 0.098 & 0.013 \\
        & mumetal & 1 & 0.0065 & 8.8e-4 \\
        \quad \quad MXC DC feedthroughs & BeCu & {100 pins} & 4.0e-5 & 5.6e-6 \\
        \quad \quad MXC RF feedthroughs & SMA & {$10\times\SI{2.3}{g}$} & 0.082 & 0.011 \\
        \quad \quad MXC RF attenuators & & {$10\times\SI{5}{g}$} & 0.0018 & 2.3e-4\\
        \quad \quad MXC isolators & & {$10\times\SI{145}{g}$} & 0.14 & 0.019 \\
        \quad \quad 4K HEMT amplifiers & & {$10\times\SI{17}{g}$} & 8.6e-4 & 1.2e-4\\
        
        %\hline
       %\quad Readout amps, etc. & resistor & {100 ct} & 1.3e-5 & 1.6e-6 \\
        \hline
        %\bottomrule
    \end{tabular}
\end{table}


\begin{table}[ht!]
    \centering
    \caption{Simulated interaction rate and dose for a silicon chip from environmental gammas, cosmic rays, and trace radioactivity inside the fridge for an unshielded system at sea level. 
    }
    \label{tab:internalrate_thresh}
    \sisetup{separate-uncertainty, table-align-uncertainty=false, table-align-exponent=false}
    \begin{tabular}{|llc|S[table-format=3.1e-1]|S[table-format=3.1e-1]|}
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        %\toprule
        \hline
        Component & Material & {Mass} & {Rate $>\SI{1}{MeV}$} & {Rate $>\SI{2}{MeV}$} \\
        & & {(kg)} & {($10^{-3}$~cts/s/g)} & {($10^{-3}$~cts/s/g)} \\
        \hline
        \multicolumn{3}{|l|}{Cosmic rays (chip horizontal)} & 0.81 & 0.15 \\
        \multicolumn{3}{|l|}{Cosmic rays (chip vertical)} & 4.0 & 0.33 \\
        \multicolumn{3}{|l|}{Ambient Gammas} & 0.25 & {$<$}0.025 \\
        \multicolumn{3}{|l|}{Ceramic PCB interposers} & & \\
        \quad  & alumina & \SI{370}{mg} & 1.5 & 1.3 \\
        \quad  & RO4350B & \SI{780}{mg} & 3.5 & 3.0 \\
        \quad  & TMM10   & \SI{550}{mg} & 7.2 & 6.1 \\
        \multicolumn{3}{|l|}{Coax connectors on package} &  &  \\
        \quad inside (line-of-sight) & SMA & {$10\times\SI{2.3}{g}$} & 26 & 20 \\
        \quad outside (no line-of-sight) & SMA & {$10\times\SI{2.3}{g}$} & 3.8e-4 & {$<$}0.01 \\
        Bump bonds & indium &{\SI{20}{\mu g}} & {$<$}1e-5 & {$<$}1e-5 \\
        \multicolumn{3}{|l|}{All other components (itemized below)} & 0.0017 & 0.0013 \\
        \hline
        \multicolumn{3}{|l|}{\quad Fridge stages and shields} & 4.4e-5 & {$<$}3e-4 \\
        \quad \quad MXC stage & Cu & 4.6 & 3.9e-7  & {$<$}3e-6 \\
        \quad \quad CP stage & Cu & 3.3 & 1.5e-7 & {$<$}2e-6 \\
        \quad \quad Still stage & Cu & 5.9 & 2.1e-8 & {$<$}3e-6 \\
        \quad \quad 4K stage & Cu & 8.7 & 1.5e-8 & {$<$}4e-6\\
        \quad \quad 50K stage & Cu & 5.1 & {$<$}2e-6 & {$<$}2e-6\\
        \quad \quad Vacuum flange & steel & 21 & {$<$}4e-5 & {$<$}4e-5\\
        \quad \quad Still can & Cu & 6.3 & 2.9e-7 & {$<$}5e-6\\
        \quad \quad 4K can & Al & 4.1 & 4.2e-6 & {$<$}9e-5\\
        \quad \quad 50K can & Al & 5.7 & 2.5e-5 & {$<$}1e-4\\
        \quad \quad Vacuum can & Al & 21 & 1.2e-5 & {$<$}3e-4 \\
        \quad \quad Gold plating & gold & 0.5 & 1.7e-6 & {$<$}2e-5\\
        \hline
        \multicolumn{3}{|l|}{\quad Experiment readout} & 0.0017 & 0.0013 \\
        \quad \quad Wirebonds & Al/Si & {$10\times\SI{0.1}{mg}$} & 1.8e-4 & 1.5e-4 \\
        \quad \quad Package & Cu & 0.1 & 0.0013 & 0.0011 \\
        \quad \quad Package Fasteners & brass & {$10\times\SI{0.3}{g}$} & 8.9e-5 & 7.5e-5 \\
        \quad \quad Cryo filters & K\&L & {$10\times\SI{15}{g}$} & 2.8e-5 & {$<$}3e-4 \\
        \quad \quad Closest coax cable & semirigid & {$10\times\SI{10}{cm}$} & {$<$}9e-9 & {$<$}9e-9 \\
        \quad \quad Coldfinger & Cu & 1.8 & 1.1e-6 & {$<$}1e-4 \\
        \quad \quad Inner shield &  &  & 1.4e-7 & {$<$}3e-3 \\
        & Cu & 1 & 1.4e-7 & {$<$}6e-5\\
        & Al & 1 & {$<$}3e-3 & {$<$}3e-3 \\
        & mumetal & 1 & {$<$}4e-5 & {$<$}4e-5 \\
        \quad \quad MXC DC feedthroughs & BeCu & {100 pins} & 9.2e-9 & {$<$}3e-8 \\
        \quad \quad MXC RF feedthroughs & SMA & {$10\times\SI{2.3}{g}$} & 4.0e-5 & {$<$}9e-5 \\
        \quad \quad MXC RF attenuators & & {$10\times\SI{5}{g}$} & 7.9e-7 & {$<$}2e-6 \\
        \quad \quad MXC isolators & & {$10\times\SI{145}{g}$} & 3.9e-5 & {$<$}1e-4 \\
        \quad \quad 4K HEMT amplifiers & & {$10\times\SI{17}{g}$} & {$<$}2e-5 & {$<$}2e-5 \\
        
        %\hline
       %\quad Readout amps, etc. & resistor & {100 ct} & 1.3e-5 & 1.6e-6 \\
        \hline
        %\bottomrule
    \end{tabular}
\end{table}


==> hitefftable.tex <==

\begin{table}
    \centering
    \caption{For a radioactive isotope (and its progeny in secular equilibrium in the case of \iso{U}{238} and \iso{Th}{232}) at a given location, average number ``hits'' depositing greater than \SI{3}{eV} in the silicon substrates per equilibrium decay (top) and average energy deposited per decay (bottom). Equivalently, conversion factors from decay rate to hit rate or dose. Values derived from Monte Carlo simulation. }
    \label{tab:hiteff}
    \begin{tabular}{l|rrrrrrr}
        \toprule
%    Source location & \iso{K}{40} & \iso{Th}{232} & \iso{U}{238} & Activation & \iso{Pb}{210} & \iso{Co}{60} & \iso{Cs}{137} \\
%    \hline \hline
%Interposer board & 1.5E+0 & 5.1E+0 & 7.1E+0 & 4.2E-1 & 1.5E+0 & 3.1E-1 & 8.2E-1 \\
%%Packge Inner Surface & 9.8E-1 & 1.8E+1 & 2.0E+1 & 9.5E-1 & 3.8E+0 & 7.8E-1 & 1.1E+0 \\
%Package & 1.3E-2 & 5.9E-2 & 7.3E-2 & 1.4E-2 & 6.8E-3 & 2.1E-2 & 9.5E-3 \\
%%Package Outer Surface & 1.1E-3 & 6.4E-3 & 6.0E-3 & 6.8E-3 & 9.0E-5 & 1.1E-2 & 3.6E-3 \\
%Experiment stage & 5.8E-5 & 1.0E-3 & 7.3E-4 & 5.2E-4 & 9.0E-7 & 9.1E-4 & 2.9E-4 \\
%Experiment shield & 1.5E-5 & 2.8E-4 & 1.9E-4 & 1.4E-4 & 0.0E+0 & 2.3E-4 & 8.1E-5 \\
%Mixing Chamber Stage & 4.5E-6 & 1.4E-4 & 1.1E-4 & 7.5E-5 & 0.0E+0 & 1.3E-4 & 4.1E-5 \\
%Cold Plate Stage & 1.1E-6 & 2.3E-5 & 1.7E-5 & 1.3E-5 & 2.1E-8 & 2.2E-5 & 6.9E-6 \\
%Still Stage & 5.4E-7 & 9.0E-6 & 7.4E-6 & 5.4E-6 & 0.0E+0 & 9.7E-6 & 2.7E-6 \\
%4K Stage & 1.7E-7 & 2.3E-6 & 1.5E-6 & 1.4E-6 & 0.0E+0 & 2.6E-6 & 4.8E-7 \\
%50K Stage & 1.9E-8 & 7.3E-7 & 4.7E-7 & 4.4E-7 & 6.3E-9 & 8.3E-7 & 2.0E-7 \\
%Vacuum Flange & 1.9E-8 & 3.4E-7 & 2.4E-7 & 2.3E-7 & 0.0E+0 & 3.8E-7 & 8.2E-8 \\
%Still Can & 3.6E-6 & 8.4E-5 & 6.9E-5 & 3.9E-5 & 0.0E+0 & 6.7E-5 & 3.3E-5 \\
%4K Can & 2.3E-6 & 3.9E-5 & 3.0E-5 & 2.1E-5 & 0.0E+0 & 3.6E-5 & 1.1E-5 \\
%Lower 50K Can & 1.9E-6 & 3.1E-5 & 2.4E-5 & 1.7E-5 & 2.1E-8 & 2.9E-5 & 9.2E-6 \\
%Upper 50K Can & 4.2E-8 & 1.4E-6 & 8.4E-7 & 8.1E-7 & 0.0E+0 & 1.5E-6 & 4.4E-7 \\
%Lower Vacuum Can & 1.6E-6 & 2.3E-5 & 1.7E-5 & 1.2E-5 & 0.0E+0 & 2.1E-5 & 7.7E-6 \\
%Upper Vacuum Can & 9.4E-8 & 9.9E-7 & 6.4E-7 & 5.7E-7 & 0.0E+0 & 1.1E-6 & 2.2E-7 \\
%\hline
        Source location & \iso{U}{238} & \iso{Th}{232} & \iso{K}{40} & Activation & \iso{Co}{60} & \iso{Cs}{137} & \iso{Pb}{210} \\        
        \midrule
        & \multicolumn{7}{c}{Hit efficiency, \si{1/g/s/Bq}} \\
        \hline
        Interposer board & 7.1E+0 & 5.1E+0 & 1.5E+0 & 3.1E-1 & 8.2E-1 & 1.5E+0 & 4.2E-1 \\ 
        %Packge Inner Surface & 2.0E+1 & 1.8E+1 & 9.8E-1 & 7.8E-1 & 1.1E+0 & 3.8E+0 & 9.5E-1 \\ 
        Package & 7.3E-2 & 5.9E-2 & 1.3E-2 & 2.1E-2 & 9.5E-3 & 6.8E-3 & 1.4E-2 \\ 
        %Package Outer Surface & 6.0E-3 & 6.4E-3 & 1.1E-3 & 1.1E-2 & 3.6E-3 & 9.0E-5 & 6.8E-3 \\ 
        Experiment stage & 7.3E-4 & 1.0E-3 & 5.8E-5 & 9.1E-4 & 2.9E-4 & 9.0E-7 & 5.2E-4 \\ 
        Experiment shield & 1.9E-4 & 2.8E-4 & 1.5E-5 & 2.3E-4 & 8.1E-5 & 0.0E+0 & 1.4E-4 \\ 
        Mixing Chamber Stage & 1.1E-4 & 1.4E-4 & 4.5E-6 & 1.3E-4 & 4.1E-5 & 0.0E+0 & 7.5E-5 \\ 
        Cold Plate Stage & 1.7E-5 & 2.3E-5 & 1.1E-6 & 2.2E-5 & 6.9E-6 & 2.1E-8 & 1.3E-5 \\ 
        Still Stage & 7.4E-6 & 9.0E-6 & 5.4E-7 & 9.7E-6 & 2.7E-6 & 0.0E+0 & 5.4E-6 \\ 
        4K Stage & 1.5E-6 & 2.3E-6 & 1.7E-7 & 2.6E-6 & 4.8E-7 & 0.0E+0 & 1.4E-6 \\ 
        50K Stage & 4.7E-7 & 7.3E-7 & 1.9E-8 & 8.3E-7 & 2.0E-7 & 6.3E-9 & 4.4E-7 \\ 
        Vacuum Flange & 2.4E-7 & 3.4E-7 & 1.9E-8 & 3.8E-7 & 8.2E-8 & 0.0E+0 & 2.3E-7 \\ 
        Still Can & 6.9E-5 & 8.4E-5 & 3.6E-6 & 6.7E-5 & 3.3E-5 & 0.0E+0 & 3.9E-5 \\ 
        4K Can & 3.0E-5 & 3.9E-5 & 2.3E-6 & 3.6E-5 & 1.1E-5 & 0.0E+0 & 2.1E-5 \\ 
        Lower 50K Can & 2.4E-5 & 3.1E-5 & 1.9E-6 & 2.9E-5 & 9.2E-6 & 2.1E-8 & 1.7E-5 \\ 
        Upper 50K Can & 8.4E-7 & 1.4E-6 & 4.2E-8 & 1.5E-6 & 4.4E-7 & 0.0E+0 & 8.1E-7 \\ 
        Lower Vacuum Can & 1.7E-5 & 2.3E-5 & 1.6E-6 & 2.1E-5 & 7.7E-6 & 0.0E+0 & 1.2E-5 \\ 
        Upper Vacuum Can & 6.4E-7 & 9.9E-7 & 9.4E-8 & 1.1E-6 & 2.2E-7 & 0.0E+0 & 5.7E-7 \\ 
        %Lead Shield & 2.8E-7 & 8.0E-7 & 7.7E-8 & ~ & ~ & 8.9E-7 & ~ \\ 
        %Lead Shield Support & 7.1E-6 & 9.4E-6 & 5.1E-7 & ~ & ~ & ~ & ~ \\ 
        %Lead Shield Top Support & 1.3E-7 & 1.7E-7 & 1.0E-8 & ~ & ~ & ~ & ~ \\ 
        \midrule
        & \multicolumn{7}{c}{Dose efficiency, \si{keV/g/s/Bq}} \\
        \hline
        Interposer board & 2.6E+3 & 2.3E+3 & 3.3E+2 & 3.7E+1 & 1.3E+2 & 4.2E+2 & 2.8E+1 \\ 
        %Packge Inner Surface & 2.3E+4 & 1.9E+4 & 1.8E+2 & 5.1E+1 & 1.1E+2 & 2.5E+3 & 3.1E+1 \\ 
        Package & 2.1E+1 & 1.8E+1 & 2.8E+0 & 3.6E+0 & 1.4E+0 & 2.2E+0 & 2.0E+0 \\ 
        %Package Outer Surface & 6.2E-1 & 8.0E-1 & 1.9E-1 & 1.9E+0 & 4.1E-1 & 1.9E-3 & 1.0E+0 \\ 
        Experiment stage & 1.0E-1 & 1.4E-1 & 1.1E-2 & 1.5E-1 & 3.4E-2 & 8.8E-6 & 7.9E-2 \\ 
        Experiment shield & 2.7E-2 & 3.5E-2 & 1.6E-3 & 3.6E-2 & 9.9E-3 & 0.0E+0 & 2.0E-2 \\ 
        Mixing Chamber Stage & 1.4E-2 & 1.7E-2 & 5.7E-4 & 2.2E-2 & 5.2E-3 & 0.0E+0 & 1.1E-2 \\ 
        Cold Plate Stage & 2.2E-3 & 2.9E-3 & 2.2E-4 & 3.2E-3 & 6.8E-4 & 1.1E-6 & 1.7E-3 \\ 
        Still Stage & 9.9E-4 & 1.2E-3 & 1.0E-4 & 1.4E-3 & 2.3E-4 & 0.0E+0 & 7.2E-4 \\ 
        4K Stage & 2.0E-4 & 3.2E-4 & 3.6E-5 & 3.7E-4 & 5.1E-5 & 0.0E+0 & 1.9E-4 \\ 
        50K Stage & 6.5E-5 & 1.0E-4 & 3.6E-6 & 1.2E-4 & 1.3E-5 & 2.7E-8 & 5.8E-5 \\ 
        Vacuum Flange & 2.8E-5 & 5.6E-5 & 1.7E-6 & 5.2E-5 & 8.5E-6 & 0.0E+0 & 2.9E-5 \\ 
        Still Can & 7.7E-3 & 1.0E-2 & 5.1E-4 & 1.2E-2 & 3.8E-3 & 0.0E+0 & 6.2E-3 \\ 
        4K Can & 3.8E-3 & 5.1E-3 & 3.4E-4 & 5.5E-3 & 1.3E-3 & 0.0E+0 & 2.9E-3 \\ 
        Lower 50K Can & 3.0E-3 & 4.4E-3 & 3.3E-4 & 4.7E-3 & 9.8E-4 & 6.3E-7 & 2.5E-3 \\ 
        Upper 50K Can & 1.0E-4 & 1.8E-4 & 8.2E-6 & 2.2E-4 & 3.9E-5 & 0.0E+0 & 1.2E-4 \\ 
        Lower Vacuum Can & 2.1E-3 & 3.1E-3 & 2.6E-4 & 3.2E-3 & 8.8E-4 & 0.0E+0 & 1.7E-3 \\ 
        Upper Vacuum Can & 8.9E-5 & 1.4E-4 & 1.4E-5 & 1.7E-4 & 2.0E-5 & 0.0E+0 & 8.3E-5 \\ 
        %Lead Shield & 3.9E-5 & 1.2E-4 & 1.0E-5 & ~ & ~ & 6.6E-5 & ~ \\ 
        %Lead Shield Support & 8.2E-4 & 1.1E-3 & 7.2E-5 & ~ & ~ & ~ & ~ \\ 
        %Lead Shield Top Support & 1.5E-5 & 2.1E-5 & 1.2E-6 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> old.tex <==
\section{Radiation shielded dilution refrigerator design}\label{sec:design}

In this section we first determine the external ionizing radiation environment we wish to shield against. From that assessment we evaluate shield designs, and arrive at a specific shielding concept.

%%%
\subsection{Quantifying the radiation environment}\label{sub:radenviro}

The first step to designing the radiation shield is to determine the background radiation environment in the shallow underground laboratory and how that radiation interacts with the devices inside the dilution refrigerator. We consider cosmic ray secondaries (muons) and gammas from decay of trace levels of radioactive material in the surrounding laboratory environment. The cosmic ray muon flux is attenuated by the overburden of the shallow underground site, but cannot be significantly further attenuated by local lead shielding. Thus, the interaction rate from cosmic ray secondary muons sets the achievable total event rate for the specific underground location. Therefore, the radiation shield design should seek to reduce the rate from the ambient gammas to a small fraction of the muon-induced rate. Section~\ref{sec:interior} will consider radioactive emissions from sources inside the shield and dilution refrigerator. We estimate that most material inside the fridge will contribute negligibly compared to cosmic ray muons, but certain commonly-used materials may be significant due to their proximity to the target device. 

The cosmic ray muon flux within the laboratory space depends strongly on the height and profile of the overburden, and the ambient gamma flux depends weakly on the materials used to construct the facility. Both the cosmic ray muon and ambient gamma fluxes are estimated by simulations normalized to measurements. Simulations were performed using the \geant{} Monte Carlo toolkit~\cite{agostinelli2003}. The laboratory considered was a simplified model of PNNL's shallow underground laboratory (SUL)~\cite{aalseth2012}. The simulated lab consists of a single room, 8~m by 8~m square floor with a 4~m high ceiling, surrounded by 1.2~m thick concrete walls and a 19~m overburden (above and extending on all sides) composed of calcium carbonate (limestone or chalk) with a density of 2.8~g/cm$^3$. The simulation geometry is shown in Figure~\ref{fig:underground}. This simplified model does not include any vertical access shafts, near which there is significantly higher muon flux, nor does it account for the ``heaped'' profile of the overburden, which affects the muon flux particularly at high zenith angles. We compensate for lack of fidelity in the simulation model by normalizing the simulated rates to measurements of cosmic ray muons taken \textit{in situ}. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/underground_model_dimensions.png}
    \caption{A \geant{} model cutaway rendering of dilution fridge (cylinders) within a concrete cavity (grey) beneath a 19~m overburden (yellow). Simulated cosmic ray secondary muon tracks are rendered in red and blue with tertiary ionized electron tracks shown in bright green.}
    \label{fig:underground}
\end{figure}

%%%
\subsubsection{Cosmic ray secondaries}\label{sub:cosmic}

%Any model estimate of the muon energy deposition rate must be calibrated against experimental reference data to ensure that assumptions used to simplify the model do not impact the results.
For this study, spectra acquired from a \SI{3}{inch} (7.62~cm) diameter and height NaI scintillation detector operated in a surface laboratory and in the shallow underground lab were  compared to simulations. The simulated detector is a NaI cylinder with \SI{3}{inch} diameter and height enclosed in a \SI{0.5}{mm} thick aluminum oxide ``reflector'' and \SI{0.8}{mm} thick aluminum case; the PMT is not modeled. The simulated detector is placed in the center of the $8\times8\times4$~m$^3$ laboratory model volume, 2.4~m from the floor. Cosmic ray secondaries are generated using the \CRY{} package~\cite{crypackage1} called from \geant{}. For the surface simulation, no walls or ceiling are modeled, and the \CRY{}-generated cosmic ray secondaries are produced from a square plane \SI{20}{m} on a side, \SI{4}{m} above the detector, which accounts for 95\% of the total cosmic ray muon flux assuming a $\cos^2\theta$ zenith angle dependence~\cite{grieder2001}. For the underground simulation, only secondary muons are generated from a \SI{38}{m} plane just at the top of the overburden (see Fig.~\ref{fig:underground}); all other cosmic ray secondary particles contribute negligibly. To speed up the simulation, we employ a biasing technique where we immediately discard before simulating any initial muon whose momentum direction points more than \SI{3}{m} from the NaI detector. This cut was tested against a full simulation with no cut and and agreed within statistical uncertainty as described in Section~\ref{sec:append-variance}. The simulated energy depositions are tallied and normalized to counts per second using the livetime reported by \CRY. 

Figure~\ref{fig:muon_validation_SUL} shows the predicted energy spectra from \geant{} compared to data acquired with a Mirion Osprey base and multichannel analyzer (92 hours at surface, 410 hours underground). A simple two-parameter fit is performed to align the measured data with simulation: a linear scale factor to convert from ADC counts to energy deposited and a linear amplitude scale. The data measured at surface agrees with the CRY-simulated rate within 20\%, which we consider reasonable agreement for comparison to an altitude, geomagnetic-latitude, and solar-cycle dependent estimate of the absolute rate of cosmic ray secondaries at any specific location on the surface of the Earth. However, the rate measured underground is more than 4 times the simulated rate, most likely due to the simplified model with flat overburden and the proximity of the measurement detector to a vertical access shaft. For the remainder of this work, all simulated underground cosmic ray rates are scaled by the obtained factor of 4.36. The measured rate underground in the 30-50 MeV peak region is reduced by a factor of 0.15 relative to surface, in good agreement with prior measurements~\cite{aalseth2012}. The excess event rate in the measured spectra below 3~MeV are from environmental gammas which were not included in these simulations. The additional, smaller excess in the surface measurements up to $\sim$\SI{12}{MeV} are most likely due to details of real cosmic ray secondary interactions with the laboratory building and detector effects such as quenching of neutron-induced scintillation, both of which were not modeled. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/naifits_surf_sul.pdf}
    \caption{Comparison of cosmic ray simulations to data collected from a \SI{3}{inch} NaI detector operated in the PNNL Shallow Underground Lab with $\sim$19~m overburden (blue, bottom) and a surface laboratory (black, top).  The spectra are linearly scaled horizontally and vertically to match the energy scale and amplitude, respectively. }
    \label{fig:muon_validation_SUL}
\end{figure}

%The fit was performed over the range 75-250 ADC counts (approximately 7.7-26 MeV). The best fit is obtained by scaling the simulated spectrum by $0.705 \pm 0.003$.


%%% POTENTIAL PARAGRAPH ADDITION: Add a paragraph break here IF we wind up using the above ground simulation text
%Details of the surface simulation comparison are provided below. We begin with discussion regarding the simulation and measurement comparison results obtained in the SUL.
%\JLO{ADD:}{Possible paragraph addition related to the above ground, RPL muon measurement, if it helps us better understand either (1) the muon simulation in SUL or (2) set a better ratio for the suppression factor for muons that can cause catastrophic error bursts.}
%\JLO{ADD:}{Add a paragraph that compares the above ground NaI measurement.}
%\JLO{ADD:}{Add a paragraph that determines from the measurement the absolute strike rate for muons. This requires integrating Figure~\ref{fig:muon_validation_SUL} from 8~MeV to 50~MeV to get the total count rate. Then, with the total count rate,divided by the PVT panel area of 76 $\times$ 76 = 5776~cm$^{2}$, and finally divide by the total run time in seconds. This muon rate will then be used in the Discussion Sec.~\ref{sec:cosmicrate} to compare to the Google Sycamore catastrophic error burst rate.}

%To validate the starting flux, we simulate the muon flux starting from a 20~m~by~20~m plane directly above the concrete ceiling, and measure the energy deposited in a muon veto panel: a 5~cm thick polyvinyltoluene (PVT) plastic scintillator paddle 76~cm on each side. The resulting spectrum, normalized to an effective livetime using the CRY toolkit, is compared to measured data from a panel of those dimensions. In order to fit the data, the simulated spectrum is convolved by a function that linearly converts from energy to arbitrary ADC units and adds a Gaussian broadening to account for the finite energy resolution of the detector. A vertical scale factor represents a correction to the CRY normalization to match the measured data livetime. The result is shown in Figure~\ref{fig:cosmicfit_surface}. The fit indicates reasonable spectral agreement above the minimum ionizing peak (below that, environmental sources dominate the measurement so we do not expect agreement). The normalization factor of 1.257 indicates that the livetime reported by the CRY toolkit is approximately 25\% too high (alternatively, the rate as calculated from the CRY toolkit is 25\% too low). 

%In order to validate the rate normalization obtained from \CRY, we compare the results of a simulation to measurements. A $76 \times 76 \times 5$~cm$^3$ PVT scintillator panel, typical for muon veto systems, was added to the simulation. Primary particles were simulated using the \CRY\ toolkit, and the resulting energy deposition spectra in the PVT panel were normalized to counts per second using the livetime as reported by \CRY. This spectrum is compared to ADC measurements for a panel of those same dimensions. For all simulations, the PVT panel is placed in an $8\times8\times4$~m$^3$ room 2.4~m from the floor. 

%For the surface comparison, the room was surrounded by 1~m concrete walls. Cosmic ray muon primaries are generated at the edge of the ``ceiling" (2.6~m from the PVT panel) in a $20\times20$~m$^2$ plane. Figure~\ref{fig:muon_validation}  shows a fit of the resulting simulation without variance reduction to 17.2~hours of data measured in the basement of the the RPL building on the PNNL campus. The only free parameters in the fit are a linear scale factor to convert energy deposited to recorded ADC counts and a scaling amplitude. The fit was performed over the range 4500-20000 ADC counts (approximately 8.9-39~MeV). The best fit is obtained by scaling the simulated spectrum by $1.257 \pm 0.003$, indicating the \CRY\ is under-reporting the rate (or equivalently over-reporting the livetime) by about 25\%. Slightly better fit results can be obtained by allowing for non-linear energy conversion or spectral broadening due to finite resolution, but these do not have significant impact on the amplitude scaling and were not applied here. The under-coverage of the simulation in the high energy region above $\sim$40~MeV most likely indicates that 20~m is an insufficient extent for primary generation at surface, as the highest energies will be from muons traversing the PVT at large oblique angles, i.e. originating far from vertically above. However, this high energy region represents only about 0.7\% of the total spectrum. 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.55\textwidth]{figures/fit_surface_20m_linear}
%    %\includegraphics[width=0.48\textwidth]{figures/fit_SUL_linear}
%    \caption{Validation of cosmic ray simulation with a PVT panel operated at surface.% (left) and in PNNL's Shallow Underground Laboratory (right).
%    }
%    \label{fig:muon_validation}
%\end{figure}

%For the shallow overburden validation, the walls were 1.2~m of concrete, and an overburden of calcium carbonate (limestone or chalk) with a density of 2.8~g/cm$^3$ extending 19~m above and to the sides of the concrete, as shown in Figure~\ref{fig:underground}. Cosmic ray muon primaries are generated just at the top of the overburden (22~m from the PVT panel) from a $38\times38$~m$^2$ plane. Figure~\ref{fig:muon_validation_SUL} shows a fit of the simulated data without variance reduction to 30 hours of data measured in the PNNL Shallow Underground Lab. The fit was performed over the range 75-250 ADC counts (approximately 7.7-26 MeV). The best fit is obtained by scaling the simulated spectrum by $0.705 \pm 0.003$.

%The effect here is opposite to that at surface: the simulated rate is higher than measured, and there is more relative weight in the simulated high-energy tail. Overall the fit is much poorer than surface. In addition to any errors present in the primary particle production,  the underground spectrum will also be influenced by inaccuracies in our definition of the overburden, which is approximate at best. In particular, there are likely differences in the material composition, density, and shape at surface (berms, etc). Nevertheless, the simulation largely agrees with measured data both at surface and underground within $\sim30\%$. %A simulation was conducted of the underground laboratory and doubling the soil density. The integral tally in the PVT panel was reduced by a factor of 2.8 indicating variations in soil density al easily encompass the observed disparity between measured and modeled data.

%%%
\subsubsection{Environmental gamma rays}\label{sub:gamma}

Estimating the ambient gamma flux followed several steps. First, we make the simplifying assumption that the gamma environment is dominated by the isotopes \iso{K}{40}, \iso{U}{238}, \iso{Th}{232} and their progeny in the concrete walls. As we will show below, this assumption agrees very well with measured data. 
The measured gamma-ray spectrum was obtained with an unshielded high purity germanium (HPGe) detector. The Mirion GC14022 HPGe detector used for these measurements was a \textit{p}-type coaxial design with a vendor-specified 140\% relative efficiency at 1.33~MeV. The detector was placed near the center of one of the SUL labs, away from walls. Collected data were analyzed using PeakEasy v4.86 to identify key terrestrial background gamma-ray emitters. The most prominent isotopes (and their decay chain) identified were \iso{K}{40}~(K), \iso{Pb}{214}~(U), \iso{Bi}{214}~(U), \iso{Ac}{228}~(Th), \iso{Pb}{212}~(Th), \iso{Bi}{212}~(Th), and \iso{Tl}{208}~(Th) which accounted for 93.5\% of the total terrestrial gamma background spectrum.

For the simulation, the identified isotopes were distributed uniformly throughout the concrete wall of the laboratory model and the characteristic gamma- and x-ray emissions were generated using \geant{}'s radioactive decay module~\cite{RDG6575161,RDG6575219}. The energy, position, and direction of each photon passing the surface of a 145\unit{cm} radius sphere centered on the HPGe were recorded. An analysis, not presented here (see Ref.~\cite{pnnl-31996}), showed the radiation emissions crossing the 145\unit{cm} radius sphere had the expected uniformity in direction angles. This permitted ``re-throwing'' (\textit{i.e.}, generation of new simulation primaries) of the gamma- and x-ray flux uniformly and isotropically from a smaller, simulated sphere inside the room. This substantially reduced the number of simulation primaries required to explore specific shield design thicknesses and event rates at the location of the superconducting devices.

%As expected, Figure~\ref{fig:gammaflux_positiondist} shows that the measured flux is uniformly distributed along the azimuthal angles and polar angles, with no strong preference for emission from any direction nor any dependence on photon energy  (\textit{i.e.}, lower-energy emitters like \iso{Pb}{212} exhibit roughly the same distribution as a higher-energy emitter like \iso{Tl}{208}). Likewise, Figure~\ref{fig:gammaflux_angulardist} shows that the measured flux is also isotropic to good approximation and with no dependence on photon energy. Because of this symmetry, we can ``re-throw'' the gamma flux originating from the walls both uniformly and isotropically from a simulated sphere inside the room and obtain similar results.

%These optimizations allow for significant speedup in simulations, as we can start the gamma-ray primaries for each simulation much closer to the volume of interest without re-transporting photons through the 1.2~m thick concrete wall upon every iteration on the shield design.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/Fluxcounter_Photon_Position_Updated.png}
%    \caption{Positional distribution of gammas emitted by radioactive decay in the concrete walls as they cross a 145\unit{cm} radius sphere in spherical coordinates.}
%    \label{fig:gammaflux_positiondist}
%     \includegraphics[width=\linewidth]{figures/Fluxcounter_Photon_Direction.png}
%    \caption{Angular distribution of gammas emitted by radioactive decay in the concrete walls as they cross a 145\unit{cm} radius sphere.}
%    \label{fig:gammaflux_angulardist}
%\end{figure}



%%%
\subsection{Simulation-driven design approach}\label{sub:simdesign}

Once we have determined the levels of contributing sources to the radiation environment in the underground laboratory, we must understand how that radiation interacts with a hypothetical superconducting qubit system. We begin by specifying the ionizing radiation sensitive superconducting devices and the metric for evaluating impact of the radiation environment. We then turn to evaluating the preferred lead shield thickness given our presumed location in PNNL's shallow underground laboratory.

We simulate a very simple model of a dilution refrigerator, loosely based on a Bluefors LD system, the dimensions of which are given in Table~\ref{tab:fridgedimensions}. We use a \dims{2}{5}{0.3}\unit{mm^3} silicon chip as a qubit substrate. Because the chance of incoming radiation interacting with such a small element is very low, in order to accumulate simulation statistics more quickly, we simulate a ``quantum computing platform'' with 144 such chips. While not representative of how superconducting qubit chips are operated in practice, we grouped nine chips together for efficiency of the radiation transport simulation. Each group of nine chips is placed on a 0.5~mm kapton ``interposer'' inside a \dims{3}{3}{2}\unit{cm^3} copper box with 0.5\unit{cm} thick sides that would act as resonating cavity and RF shielding package for typical microwave-addressed qubits. Sixteen of these units are attached to a 1/4'' (6.35~mm) thick copper plate, 18~cm per side, hanging vertically from the dilution refrigerator mixing chamber stage. The simulated package can be rotated in the simulation so that the qubits are oriented either horizontally or vertically, which affects interaction rate with the strongly-directional cosmic ray muon flux. Figure~\ref{fig:simcomputer} shows the fridge and chip layout.

\begin{table}[ht!]
    \centering
    \caption{Dimensions of stages and cans for the simulated dilution refrigerator. All dimensions are in millimeters. All copper materials are assumed to be gold-plated. For simplicity in the simulation, gold-plated copper is modeled as copper with 0.1\% bulk admixture of gold.}
    \label{tab:fridgedimensions}
    \begin{tabular}{|l|ccccl|}
    \multicolumn{6}{l}{\vspace{-0.75em}} \\
    \multicolumn{6}{l}{\textbf{Cooling stages}} \\ 
    \hline
    Stage & Vertical Offset & Radius & Thickness & & Material \\ 
    \hline
    Vacuum Flange & 0 & 261 & 12 & & stainless steel \\
    50K           & 191 & 223.5 & 12 & & aluminum \\
    4K            & 480 & 176 & 10 & & copper \\
    Still         & 730 & 153 & 9 & & copper \\
    Cold Plate    & 829 & 140 & 6 & & copper \\
    Mixing Chamber & 997 & 142.3 & 8 & & copper \\
    \hline
    \multicolumn{6}{l}{\vspace{-0.75em}} \\
    \multicolumn{6}{l}{\textbf{Cans}} \\
    \hline
    Can & Vertical Offset & Radius & Height & Thickness & Material \\
    \hline
    Vacuum top & 12 & 230 & 486 & 3.2 & aluminum \\
    Vacuum bottom & 498 & 207.65 & 840 & 3.2 & aluminum \\
    50K top & 203 & 204 & 286.5 & 1 & aluminum \\
    50K bottom & 489.5 & 182 & 793 & 1 & aluminum \\
    4K & 490 & 160 & 774 & 1.5 & aluminum \\
    %Still & -- & -- & -- & -- & -- \\
    Mixing Chamber & 739 & 151.5 & 500 & 0.5 & copper \\
    \hline
    \end{tabular}
\end{table}

\begin{figure}[ht!]
    \centering
    %\includegraphics[width=0.4\textwidth]{figures/fulldrcutaway.png}
    \includegraphics[width=0.5\textwidth]{figures/g4_fridge_slice.png}
    \caption{Cutaway view of the dilution refrigerator simulated in \geant{}. showing the quantum computing platform with 16 device packages, each housing 9 silicon qubit chips.}
    \label{fig:simcomputer}
\end{figure}

For each radiation source (cosmic ray muons and ambient gammas), we calculate two quantities for the qubit chips: interaction rate and absorbed dose per unit mass. For gammas, the interaction rate is calculated as the number of recorded interactions per primary photon, multiplied by the photon flux calculated in Section~\ref{sub:gamma}, and finally multiplied by the area of the surface from which the gammas are re-thrown, as described above. For cosmic rays, the interaction rate is the number of recorded interactions divided the livetime as reported by the CRY toolkit and scaled by the factor of 4.36 obtained in Section~\ref{sub:cosmic} required to match measured data. In both cases, dose is equal to the interaction rate times the average energy deposited per interaction. 
%Reporting results using both of these metrics is primarily for making historical comparisons.

If qubit disturbance is driven by prompt quasiparticle bursts coincident with radiation interactions~\cite{cardani2021,mcewen2022}, the total amount of energy deposited may not be relevant if above a minimum threshold. That is, if there is a minimum threshold of injected energy which causes a substantial quasiparticle density increase at the Josephson junctions that will result in rapid qubit decoherence, then the key feature is the interaction \emph{rate}. In such interaction rate-driven scenarios, qubit disturbance would be expected to have a direct (linear) relationship with the interaction rate. However, if the radiation dose is the more important variable, as might be the case if some fraction of the energy input goes into the creation of a long-lived excitation, then the qubit disturbance mechanism would be expected to scale with the energy input, possibly nonlinearly, following a nonequilibrium quasiparticle density model~\cite{vepsalainen2020}. Understanding the applicability of these two scenarios is an on-going area of investigation. For utility, we will present both interaction rate and dose estimates. %\footnote{\JLO{JLO:}{We could add a sentence to the end of this paragraph about how we think, or this UG DR design implies, a interaction rate metric is more appropriate for our studies. I tried a couple such statements and they all felt ``premature'' for this stage of the document.}}

Cosmic rays, which interact more rarely but deposit more average energy when the chips are oriented vertically, have a higher dose rate relative to gammas, and so in practice the shield design is driven by the interaction rate metric, since that produces the more stringent requirement. In other words, in an unshielded system, gamma rays account for the majority of the count rate, but a smaller fraction of the total dose, so the shield's effectiveness on dose rate hits diminishing returns sooner. Thus, we will use interaction rate as a primary metric for shield design evaluation. Consistent with the above description for the interaction rate metric, we use units of counts/s/g. For a thin, square silicon chip placed in a uniform, isotropic gamma- and x-ray radiation environment, the orientation is unimportant. However, the silicon chip's orientation , vertical or horizontal, and aspect ratio impact the interpretation of muon interaction rates measured in units of counts/s/g. Given the single simulation model used throughout this report, relative comparisons are valid, but we caution readers from directly attributing the counts/s/g rates we calculate for muons to their local systems.

Simulations to guide the shield design proceeded in three stages. First, we simulate cosmic rays and ambient gammas interacting with our model dilution refrigerator and qubit substrates, without any shielding. This determines the required attenuation factor to bring the rate from gammas down to a fraction of that from cosmic rays. We then add an idealized, hermetic lead shield model around the dilution refrigerator and vary the thickness until sufficient gamma-ray reduction is achieved. Finally, we add more realism to the shield model, accounting for reductions in the shield's effectiveness due to \textit{e.g.} mechanical supports and interfaces, penetrations for cooling and signal lines, and gaps from finite mechanical tolerances. Results from this final stage inform the specifications for the shield's engineering design.

%%%
\subsection{Lead shield design evaluation}\label{sub:shield}

To simplify the large possible parameter space for the specific shield design, we assume the shield is built primarily from ``standard'' \dims{2}{4}{8}\unit{inch^3} bricks. This sets a natural step size for considering thickness variations. We also use this assumption to simplify modeling gaps in the shield to set extremely conservative tolerances (\textit{i.e.}, the possibility for gaps between lead shield bricks). In the simulation, bricks are arranged with an edge parallel to the shield's thickness, such that any gaps between bricks become direct ``holes'' in the shield. We then add gaps of the specified tolerance around each individual brick and evaluate the effect. In the actual design, the bricks are ideally arranged with overlapping gaps to prevent such direct lines of sight, and the only full gaps would be at the ``seams'' where movable sections meet. These full gaps are mitigated in the design with stepped faces at the seams. 

Figure~\ref{fig:specvsshieldthick} shows the simulated spectrum of ionizing interactions in the silicon substrates for cosmic rays and for the ambient gamma flux as a function of the thickness of an idealized hermetic lead shield. Table~\ref{tab:ratevsshieldthick} and Figure~\ref{fig:ratevsshieldthick} summarize the results. As discussed previously, the details of the overburden profile affect the cosmic ray angular distribution and therefore the spectrum in the silicon. In particular, more flux at higher zenith angle (closer to the horizon), which is likely the case in the PNNL SUL, would lead to higher average energy deposition for horizontally-oriented chips and conversely lower average energy deposited for vertically-oriented chips.  The total ionizing radiation interaction rate decreases with additional shielding, but with significantly diminishing returns as the residual gamma rate becomes much less than the cosmic ray rate. With 4\unit{inches} of lead shielding, the simulated gamma rate reaches about 2\% of the cosmic ray rate for a vertically-oriented chip, which we deem an acceptable compromise. %\footnote{\JLO{NOTE: }{There was some analysis of adding an additional 2'' (5.08~cm) of lead, but the presentation was a bit confusing. However, the paragraph's final sentence makes the real point about when a thicker shield is worthwhile.}} 
%However, given the $\sim\pm25\%$ uncertainty in the cosmic ray rate from comparisons to PVT detectors, additional shielding might be desired to ensure the devices reach the maximum potential.
%(Taking our best estimate for cosmic ray interaction rate, 
%For the 19~m overburden we simulated, an additional 2\unit{inches} of shielding would reduce the {\em total} rate by roughly 9\%. 
%If the cosmic ray rate is actually 30\% lower, the additional marginal reduction would be $\sim14\%$.)
For deeper sites with more overburden, sufficient to reduce the cosmic ray rate by an additional factor of $\sim$10, additional lead shielding would be warranted (assuming the same concrete-originated gamma-ray environment).

\begin{figure}[ht!]
    \centering
    %\includegraphics[width=0.9\textwidth]{figures/spectrum_onecan.pdf}
    \includegraphics[width=0.9\textwidth]{figures/radfridgepaper_radspectra.pdf}
    \caption{Simulated spectrum of ionizing interactions in the silicon substrates for cosmic rays and for the ambient gamma flux as a function of the thickness of an idealized hermetic lead shield, and for the shield with penetrations described in \protect{Section~\ref{sub:shield}}. 
    %The cosmic ray spectrum is scaled by a factor of 4.36 obtained by the best fit of simulated muon spectra to data in an NaI detector in the SUL (Fig~\protect{\ref{fig:muon_validation_SUL}})
    %\BML{BML}{Should we just drop this figure?  It shows that the cosmic ray spectrum depends a lot on chip orientation, BUT due to poor modeling of the overburden I doni't trust it to be particularly accurate (e.g. for a non-flat overburden I would expect more high energy for a horizontal chip. In other words, taking the flat overburden sim and scaling does a good job modeling the NaI data, but it has a 1:1 aspect ratio; it's a much poorer approximation for chips} \JLO{JLO:}{Keep the figure. Add some language about how the no flat overburden might alter the spectra shape, but the primary rate and shapes should be appropriately representative.} \JLO{JLO:}{Recall, we also wish to make a comment about hot eh cosmic ray ``peak'' in the chip is at lower energy in contrast to gammas that dominate at higher energy depositions.}
    }
    \label{fig:specvsshieldthick}
\end{figure}

\begin{figure}[ht!]
    \centering
    %first label: bare fridge no shield
    %\includegraphics[width=0.9\textwidth]{figures/ratevsshield.pdf}
    \includegraphics[width=0.9\textwidth]{figures/radfridgepaper_ratevshield.pdf}
    %\missingfigure{rate vs shield thick}
    \caption{Simulated interaction rate (solid black, left axis) and dose rate (dashed blue, right axis) of ambient gammas as a function of shield thickness for an idealized hermetic lead shield. Hit rates and doses for cosmic rays in the PNNL Shallow Underground Laboratory for a vertically-mounted chip (dashed red line) and the gamma rates for the shield described in \protect{Section~\ref{sub:shield}} (magenta) are also shown. Points are slightly horizontally staggered to improve readability. The vertical axes are arranged so that the cosmic ray and ``this work'' points are correct on both axes. }
    \label{fig:ratevsshieldthick}
\end{figure}

\begin{table}[ht!]
    \centering
    \sisetup{separate-uncertainty, table-format=3.3(1)}
    \begin{tabular}{l|SS}
        \toprule
        Source, Configuration & {Interaction rate} & {Dose rate} \\
        & {(10$^{-3}$ counts/s/g)} & {(keV/s/g)} \\
        \midrule
        %cosmic rays & 5.07(5) & 1.65(2) \\ %not scaled 
        Cosmic rays, Chip vertical & 23.1(3) & 7.2(1) \\
        Cosmic rays, Chip horizontal & 44.1(4) & 6.89(8) \\
        \hline
        Gammas, No lead shield & 417(2) & 53.6(4)\\
        Gammas, 2'' (5.08~cm) hermetic lead shield & 11.3(3) & 2.04(9) \\
        Gammas, 4'' (10.16~cm) hermetic lead shield & 0.54(8) & 0.10(2) \\
        Gammas, 6'' (15.24~cm) hermetic lead shield & 0.04(2) & 0.010(5) \\
        \hline
        %Gammas, detailed shield & 0.75(6) & 0.12(1)\\
        %Gammas, detailed shield with 1\unit{mm} gaps & 1.0(1) & 0.14(2)\\
        Gammas, 4'' (10.16~cm) detailed lead shield & 0.80(9) & 0.13(2) \\
        \bottomrule
        %with 3\unit{mm} gaps & & \\
    \end{tabular}
    \caption{Simulated interaction rate and dose in silicon chips from cosmic ray and ambient gamma sources vs. various design configurations. The final detailed shield includes expected holes in the shield for cryogenic and power service (see text body). Uncertainties are derived from simulation statistics only. Table data are plotted in \protect{Fig.~\ref{fig:ratevsshieldthick}}.}
    \label{tab:ratevsshieldthick}
\end{table}

%\subsubsection{Mechanical design}\label{sub:shield}
%\todo[inline]{Add text describing the design in general (top/bottom sections, as close to the fridge as possible, bottom section slides on rails to allow access, top is fixed and supported by vendor frame, etc.) }

Simulating a monolithic shield without penetrations, gaps, or imperfections is computationally convenient but unrealistic. This study also considered the mechanical limitations on shield coverage by including necessary perforations for the helium lines, experimental connections, mechanical maintenance, and loading limitations of the DR. The shield design presented in Figure \ref{fig:cad_fridge} takes into account these realistic requirements. The shield is split into bottom and top sections to accommodate the section of frame from which the dilution refrigerator hangs. The top is further split into two sections, an upper ``roof'' and a lower ``skirt'', with the gap between allowing for the fridge helium and vacuum connections as well as experiment cabling. The shield bottom consists of a single fixed wall attached to the DR frame, with the other four sides mounted to a linear motion system that allows access to the cans and interior space and enables rapid shielded vs.\ unshielded comparison measurements. The lead is stepped where the two parts of the bottom shield meet to prevent line-of-sight gaps. The shield is designed to be constructed from ``standard'' \dims{2}{4}{8}\unit{inch^3} lead bricks, with a small number of half-size bricks. This allows the bricks to be stacked by hand during initial assembly. Once stacked, the bricks will be held in place by aluminum sheets anchored to the frames. 

\begin{figure}[ht!]
    \centering
    %\includegraphics[width=0.48\textwidth]{figures/shieldisoclosed.png}
    %\includegraphics[width=0.48\textwidth]{figures/shieldisoopen.png}
    %\includegraphics[width=0.48\textwidth]{figures/shieldcutawayclosed.png}
    %\includegraphics[width=0.47\textwidth]{figures/shieldcutawayopen.png}
    %\includegraphics[width=0.75\textwidth]{figures/DilFridgeModel10.JPG}
    \includegraphics[width=0.48\textwidth, trim=300 20 300 20, clip]{figures/Dil Fridge Model 13.JPG}
    \includegraphics[width=0.48\textwidth, trim=300 20 300 20, clip]{figures/Dil Fridge Model 12.JPG}
    \caption{Draft renderings of the lead shield around the dilution refrigerator in open (left) and closed with cutaway (right) configurations.} 
    \label{fig:cad_fridge}
\end{figure}

%\textbf{OPTIONAL PARAGRAPH:}
%The bottom shield forms a five-sided, open-topped ``box,'' split into two sections: a single immovable wall, and a sliding ``door'' section for the bottom and remaining three sides that allows access to the refrigerator. When closed, the bottom section exterior dimensions are $32\times 34$~inches by 52~inches high; each section is four inches thick. The fixed section is attached to and supported by the fridge frame. The whole assembly is shifted approximately two inches off the center of the fridge in the direction of the fixed section to allow access to the bolts on the top flange. The door section of the shield is held by a sturdy structure of aluminum extruded frame pieces, aluminum gussets, and aluminum plates. The door section contains an estimated 8100 pounds (3674 kg) of lead with a total estimated weight of 8820 pounds (4000 kg). The fixed section contains 2635 pounds (1195 kg) of lead and a total estimated weight of 3000 pounds (1360 kg). The door structure is mounted to a linear ball bearing system with a dynamic load capacity of 3800 pounds (1720 kg) that ride on two steel shafts mounted to support rails which are mounted to an aluminum plate. The door has six ball-bearing blocks to maintain a greater than 2.5 factor of safety. The door is moved by a motorized linear screw system to maintain minimal lateral momentum.

%\textbf{OPTIONAL PARAGRAPH:}
%Shielding on top the frame is also divided into two sections, arranged in a square ``top hat,'' with the $40\times40$~inch, 8~inch wide ``brim'' around the edge of the plate from which the fridge hangs, and the $32\times32$~inch top on a raised platform covering the center, overlapping the brim by four inches. The $\sim8$~inch gap between the brim and top of the upper shield allow for plumbing and cabling. The fridge frame is reinforced to bear the additional lead weight. The arrangement of the top layers prevents any direct line-of-sight to the fridge experiment space. Supports are added to the legs of the frame and mounted to the floor or aluminum plated supporting the door sections of the shield. Estimated total weight of the cryostat (330 pounds or 150 kg), lead (4400 pounds or 2000 kg), external components (500 pounds or 227 kg), and internal components (300 pounds or 136 kg) is 5530 pounds (2513 kg). The frame is capable of supporting the estimated total weight of all estimated materials and components with a factor of safety well above 10. The frame is anchored to the laboratory wall (on the fixed bottom side) to stabilize the entire system in the event of seismic activity. 

Table~\ref{tab:ratevsshieldthick} lists the ionizing radiation interaction rate and dose for several shields considered in this work. The open sections of the shield described above increase the interaction rate (absorbed dose) from ambient gammas by 50\% (30\%) as compared to an idealized hermetic 4'' (10.16~cm)) shield. Not shown is the effect of adding a 1\unit{mm} gap around every brick in the shield (with bricks place parallel to the shield's thickness), which would increase the interaction rate (dose) by another 30\% (20\%). Since even this extremely conservative estimate of the contribution from gaps is minimal, we are comfortable stating that a 1\unit{mm} ($\sim$1/16'') tolerance for all gaps in the shield should be sufficient. The simulation can also be configured to evaluate specific gap tolerances, such as the ``seam'' where the two moving parts of the bottom part of the shield meet. However, since that particular seam does not have direct line-of-sight to the sensitive elements, we neglect it. 


%%%
%%% Interior
%%%

\section{Interior radiation environment}\label{sec:interior}

%%%
%\subsection{Interior materials and instrumentation}\label{sub:dr}

With a notional shield thickness selected based upon comparison to the cosmic ray interactions, we can turn to evaluating whether the materials internal to the shield spoil the desired benefit of the lead shield. The radiation emissions from a number of sources are considered. We begin by considering radioactivity in the lead itself and the aluminum framing used in the design. We then move on to investigating trace radioactive isotopes present in the dilution refrigerator materials. In particular, we present an assay of the trace levels of radioactive contaminants of three qubit devices. Finally, we consider the instrumentation required to operate superconducting devices, again with specific reference to superconducting qubits.

%A range of materials may be considered as common materials used in a dilution refrigerator. These materials include: stainless steel, copper, brass, bronze, Kapton, teflon, delrin, viton, indium vacuum seals, silver solder, vacuum grease, Cu-Ni supports, ceramics, Be-Cu pins etc$\ldots$. \textbf{It is odd we make this list and then ignore it. Need to fix this.} However, not all components generate enough radiation in proximity of the qubits to impact them. More to the point, the arrangement of subsidiary materials will be highly experiment-dependent.

%%%
\subsection{Shield and refrigerator}\label{sub:shieldandfridge}

To fully specify the physical model for simulating radiation transport in the immediate environment of the superconducting qubits, the bulk construction materials of the shield and dilution refrigerator must be included. This includes consideration of the lead shield, any aluminum framing or barriers inside the lead, and copper or stainless steel used in the dilution refrigerator construction. In most cases, the refined materials (metals, polymers, etc.) used in the dilution refrigerator construction have substantially lower levels of trace radioactivity than the surrounding laboratory, hence the utility of the lead shield.

There are two two primary considerations in adding these bulk construction materials to the physical model. First, dense materials or materials with substantial mass impact the attenuation of gamma ray radiation inside the shield and therefore must be present within the model for realistic radiation transport simulation. Second, the materials themselves contribute to the ionizing radiation environment within the shield due to the presence of naturally occurring radioactive contaminants found in all materials. These materials define the ultimate limit of how low in radioactive background can be achieved while using an ``off-the-shelf'' dilution refrigerator; further gains would require a custom design using specifically low-background materials. 
%We will evaluate superconducting device-specific instrumentation separately in Sec.~\ref{sub:drinstrum}, as their ionizing radiation impact can largely be evaluated without modifying the physical model described in this section.

Table~\ref{tab:radiopurity_lvls} lists the assumed levels of specific activity of different radioactive contaminants in the materials considered for this estimate. The lead is assumed to be modern lead (\textit{e.g.}, mined and processed within the last $\sim$60 years), which has been shown to have substantial \iso{Pb}{210} activity compared to ancient lead (\textit{e.g.}, Roman lead)~\cite{Keillor2017185, Orrell20161271}, largely due the 22.3~year half-life of \iso{Pb}{210}. The major components of a dilution refrigerator also contain trace quantities of primordial radioactivity, predominantly from $^{40}$K, $^{238/235}$U, and $^{232}$Th. In addition to these environmental contaminants modern sources of steel and copper have $^{60}$Co, respectively from recycling contamination in the cobalt used for steel production and as a result of cosmogenic spallation processes in copper.
%\footnote{\JLO{Modern Myth:}{That nuclear weapon testing is \emph{the} reason for \iso{Co}{60} contamination}} 

%Here we consider only the elements of the shield and dilution refrigerator itself (cooling stages and cans) and the typical isotopes of concern listed in Table~\ref{tab:radiopurity_lvls}.

\begin{comment}
\begin{table}
    \centering
    \caption{Radio-contaminant levels used to normalize the simulated dose per disintegration using GEANT4. \JLO{}{Review the choice of Pb-210 contamination to use.}}
    \label{tab:radiopurity_lvls}
    \begin{tabular}{l|ccccccc|c}
    & \multicolumn{7}{c|}{Isotope concentrations (mBq/kg)} & \\
    Material   & $^{238}$U & $^{235}$U & $^{232}$Th & $^{210}$Pb & $^{137}$Cs & $^{60}$Co & $^{40}$K & Ref. \\ \hline
    lead       &  $<$0.03   & --      & 2      & \JLO{}{$4\times10^4$} & --      & --     & --     & \cite{Orrell20161271, Keillor2017185} \\
    copper     &   11       & 0.47    & 0.37   & 40            &  0.14   & 0.24   & 1.3    & \cite{aprile2011a} \\
    steel      &   130      & 2       & 2.4    & --            &  0.9    & 8.5    & 10     & \cite{aprile2011a} \\
    aluminum   &   66       & 2.64    & 200    & --            & --      &  --    &  2100  & \cite{leonard2008a} \\
    gold       &   74.4     & 3       & 18.5   & --            & --      &  --    & 146    & \cite{leonard2008a, abgrall2016} \\
    \end{tabular}
\end{table}
\end{comment}



    
%        



%%%
\subsection{Interior instrumentation}\label{sub:drinstrum}

Up to this point our description has generally progressed from outer most to inner most regions of consideration, beginning with considering cosmic rays and, in the last subsection, the shielding and dilution refrigerator materials. In this subsection we invert that approach and look at the trace radioactivity present in device-specific instrumentation hardware, starting with, in our case, superconducting qubit devices and working outward. 
%\JLO{Ben check this:}{In most all cases the physical model used for radiation transport simulation no longer needs modification.} 
The evaluation process will consider ionizing radiation sources nearest, and then progressively further away, from the qubits.  As a technical detail, we do not implement details of components like coax cables and connectors to the radiation transport simulation. Rather, we use already-defined elements to approximate their location. For example, coax cables connecting the device package to the mixing chamber plate are treated as uniformly spread across the experiment stage, and likewise connectors on the MXC plate are treated as uniformly distributed throughout the simulated MXC plate volume.

\paragraph{Qubit fabrication}


\paragraph{Qubit isotopic assay}


\paragraph{Refrigerator and qubit instrumentation}
%\JLO{Rewrite: }{The dilution refrigerator and instrumentation to operate superconducting qubits typically consists of wire bonds, interposer boards for supporting qubit chips, signal/readout connectors, device packaging, coaxial RF cables, RF transfer or conditioning components, and feedthroughs. These were listed roughly ordered from the cold stage up to room temperature. To determine a trace radioactive content load, at the appropriate locations in the dilution refrigerator, Table~\ref{tab:radiopurity_lvls_inst} presents from coldest to warmest, the various instrumentation stages, noting the main materials and masses for each stage of instrumentation.}

The qubit devices are located at the coldest stage of a dilution refrigerator surrounded by components and instrumentation that enable quantum-coherent operation of superconducting circuits. We focus on the activity of the materials that are nearest to the qubits: the device package, electrical interconnects, and the shielding enclosure.

As previously mentioned, the qubit devices are made of superconducting thin films patterned on high quality dielectric substrates such as silicon and sapphire, which typically have a substrate area of $\sim\!10\,\mathrm{mm}^2-250\,\mathrm{mm}^2$ and a $\lesssim1\,\mathrm{mm}$ thickness. Since the qubit devices themselves have appreciable radiopurity, we have not included these materials in Table~\ref{tab:radiopurity_lvls}. While most qubit devices are fabricated as a single chip, some qubit processors device are implemented with a multi-chip architecture which use additional materials also not included in Table~\ref{tab:radiopurity_lvls}, such as indium bump-bonds.

We note in passing that indium is naturally radioactive, specifically isotope $^{115}$In with $\sim$96\% natural abundance that emits a relatively energetic beta emission with an endpoint energy of 497~keV, decaying to the ground state of stable $^{115}$Sn, without appreciable gamma-ray emission. Natural indium has a specific activity of approximately 0.25~Bq/g which is to be compared with the mass of individual indium 4000~$\mu$m$^3$ bump-bonds~\cite{Broennimann_2006} of $\sim$3$\times$10$^8$~g. A case of 10,000 indium bumpbonds would produce one beta emission approximately every four hours.
%\footnote{\JLO{Math notes:}{Specific activity = N$_A$ $\times$ ln~2 / (T$_{1/2}$ $\times$ M), where T$_{1/2}$ = 4.41$\times$10$^{14}$~y for In-115 and M = 115 for In-115 or 114.8 for natural indium. The citation given says a indium bump bond is 4000~$\mu$m$^3$ or 4$\times$10$^{-9}$~cm$^3$, which for a density of 7.31~g/cm$^3$ converts to a mass\ldots and then I get to one decay every 4~hours.}}

The qubit devices are housed in a machined package enclosure typically made of oxygen free high purity copper (OFHC) or aluminum. Inside the device package, the qubit chip is often placed on a microwave interposer that is often made from ceramic materials but could also be high purity crystalline dielectric. The purpose of the interposer is to secure (and thermalize) the qubit chip while providing routing for electrical signals between the device and wiring connections. The qubit device chip is wirebonded, possibly bumpbonded, to the interposer and usually at the center of the package. Adhesives such as GE varnish or silver paste are sometimes used to secure the qubit device in place and improve thermalization, although this can be achieved by wirebonds alone. Although the level of radioactivity in epoxies can vary significantly, we neglect to model them due to the very small mass used for these applications. 
%While GE varnish activity levels are \note{[...]} the radioactivity of silver paste is \note{[...]} \cite{Busto:2002hq, cardani2021}. \BML{}{Fill in this info}

The bulk material of the package interposer is a mineral composite that partially surrounds the device chip. The interposer has metallization layers that are gold, copper, tin, or aluminum. Typical choices for the interposer bulk material include Rogers TMM10, Rogers ``RO series'', and alumina. As a general rule, ceramics often have above-average levels of radioactivity. This, coupled with their close proximity to the qubit, leads to the conclusion that the interposer may be a significant source of radiation events. In Table~\ref{tab:hpge_pcb_results}, we report the radionuclide assay of samples of Rogers TMM10 and RO4350B PCB substrates, each counted for approximately 5 days on a high purity germanium system. As can be seen in Table~\ref{tab:radiopurity_lvls}, these ceramic and alumina substrates do indeed have substantially higher levels of radioactivity than other materials in the dilution refrigerator. FR4, another common PCB substrate, has similar high levels of radioactivity~\cite{cardani2023, ARMENGAUD20131}.

\begin{table}[ht!]
    \centering
    \caption{Radioactive contaminants in Bq/kg measured in Rogers ceramic PCBs by HPGe counting. Only isotopes identifed with $>$90\% confidence are reported. The uncertainty in the final digit is reported in parentheses.}
    \label{tab:hpge_pcb_results}
    \sisetup{table-format=2.1(1)}
    \begin{tabular}{lc|SSSSSSS}
        \toprule
        Sample & Mass & {\iso{K}{40}} & {\iso{Tl}{208}} & {\iso{Pb}{212}} & {\iso{Bi}{214}} & {\iso{Pb}{214}} & {\iso{Ra}{226}} & {\iso{Pb}{210}} \\ 
        \midrule
         TMM10 & \SI{200}{g} & 17.3 \pm 0.9 & 1.51 \pm 0.06 & 5.5 \pm 0.3 & 28.9 \pm 0.4 & 25.4 \pm 0.8 & 29 \pm 2 & {-} \\
         RO4350B & \SI{30}{g} & 9.1 \pm 0.8 & 4.9 \pm 0.2 & 15.1 \pm 0.9 & {-} & 11.2 \pm 0.4 & 8 \pm 4 & 11 \pm 2 \\
        \bottomrule
    \end{tabular}
\end{table}

Since the superconducting qubits are sensitive to magnetic fields, non-magnetic materials are selected for the package and nearby interconnects instead of equivalent ferromagnetic components. Device packages usually have non-magnetic (BeCu) coaxial connectors attached to the package perimeter. The coaxial cables that mate to these package connectors are also selected as non-magnetic. The proximity and significant potential activity of BeCu (Table~\ref{tab:radiopurity_qubits}) make these items of concern. We assayed four SMA connectors (in two batches) as well as three sections of an RG405 coax cable (with braided tinned copper outer conductor) using the dissolution and ICP-MS technique described above. Before dissolution, the cables and connectors were cleaned by sonication at room temperature, first with a 2\% Micro90 solution, then MilliQ water, for 15 minutes each with a triple rince in MilliQ water after each sonication step. 

may limit physical qubit coherence. In addition to BeCu, package connectors may also include a ceramic or glass component that could contribute substantial activity.

At the coldest cryostat stage, the qubit package is fastened to a copper mounting fixture that is well-thermalized to the mixing chamber of the dilution refrigerator. We note that the qubit chip is commonly mounted with a vertical orientation for reasons of convenience, which approximately doubles the average absorption of energy per interaction from cosmic rays compared to a horizontally orientated qubit chip (\textit{e.g.}, see Fig.~\ref{fig:specvsshieldthick}). 

The device package and mounting fixture is enclosed in an ``experiment shield'' which consists of multiple metal shields that isolate of the qubit device from electromagnetic radiation and magnetic field noise. These shields are made of tin-plated copper, aluminum, and high permeability alloys such as Cryoperm or mumetal. The aluminum alloy 6061 is commonly used for its machinability. Both mumetal (magnetic shielding) and particularly aluminum have typical levels of radioactivity orders of magnitude higher than copper as shown in Table~\ref{tab:radiopurity_lvls}. The innermost shield is sometimes coated with black paint (eg. \textit{Berkeley black}), to act as an absorber of stray electromagnetic radiation. Paints often have high radioactivity, on the order of Bq/kg~\cite{lawson2011}, and may contribute similar amounts to the radiation budget as the aluminum shield even with much lower overall mass.  
%Likewise, we expect similar levels of activity from Eccosorb, used in dissipative filters, and the epoxy Stycast 2850FT, commonly found in cryogenic setups \cite{Busto:2002hq}. \note{[Please edit/correct this statement as needed]} \BML{}{Fill in missing info here}

The cryogenic components outside the ``experiment shield'' comprise similar materials, and activity, as the materials we have addressed. The specific composition of these components and instrumentation at warmer stages are considered relatively insignificant compared to the materials proximate to the qubit device. While materials in a cryogenic setup are typically selected for their structural, electrical, and thermal properties, this investigation suggests that selective replacement of the most influential components, such the package interposer and connectors will likely mitigate radioactivity backgrounds for superconducting qubits. 


\begin{comment}
\BML{BML}{hide this table so the result table doesn't get pushed off}
\begin{sidewaystable}[ht!]
    \centering
    \caption{Typical radiopurity of various materials. ILIAS Database \url{http://radiopurity.in2p3.fr/}. * Special in some way. ** Rough average of XENON SMD resistors. }
    \label{tab:assays}
    \begin{tabular}{lclrrrrrrr}
    \hline
    Label & Ref & Note & U238 & Th232 & K40 & Activation & Co60 & Cs137 & Pb210 \\
    \hline
copper & & & 1.10E-02 & 3.70E-04 & 1.30E-03 & 6.61E-03 & 2.40E-04 & 1.40E-04 & 4.00E-02 \\
steel & & & 1.30E-01 & 2.40E-03 & 1.00E-02 & & 8.50E-03 & 9.00E-04 & \\
aluminum & & & 6.60E-02 & 2.00E-01 & 2.10E+00 &  &  &  & \\
gold & & & 7.44E-02 & 1.85E-02 & 1.46E-01 &  &  &  & \\
lead & & & 3.00E-05 & 2.00E-03 & & & & & 400 \\
\hline
BeCu wire & \cite{leonard2008a} & & 22.22222222 & 1.504065041 & 1.54799E-05 & 6.61E-03 & & & 4.00E-02 \\
cirlex & \cite{aprile2017a} & & 8.10811E-05 & 2.48649E-05 & 0.000178378 & & 5.2973E-06 & 6.48649E-06 & \\
mmcx * & \cite{aprile2017a} & per pair, 442g & 4.40E-04 & 3.80E-05 & 1.80E-04 & & 3.80E-06 & 3.30E-06 & \\
RG174 * & \cite{aprile2011a} & per meter & 1.80E-04 & 2.00E-05 & 2.00E-04 & & 3.90E-06 & 1.20E-05 & \\
RG196 & \cite{aprile2017a} & & 1.90E-03 & 7.70E-04 & 9.00E-03 & &  2.70E-04 & 4.10E-04 & \\
kapton & \cite{aprile2017a} & & 1.00E-01 & 4.00E-04 & 3.90E-01 & & 4.60E-03 & 1.60E-02 & \\
Al-Si bonding wire & \cite{abgrall2016} & & 0.107407407 & 0.369918699 & 0.101547988 & & & & \\
brass & \cite{ARMENGAUD20131} & & 4.90E-03 & $<$3.00E-03 & $<$4.00E-02 & $<$6.61E-03 & & & $<$4.00E-02 \\
mumetal & ILIAS & & 2.00E-02 & 7.00E-03 & 1.50E-02 & & & & \\
delrin & LRT 2010 & & 2.52E-03 & 2.74E-03 & 1.14E-02 & & & & \\
d-sub pins * & & per par & 2.20E-06 & 7.10E-07 & & & & & \\
ceramic feedthrough & \cite{aprile2011a} & cabum-MDC & 1.30E-02 & 1.80E-02 & 4.90E-02 & & 2.10E-02 & 5.00E-03 & \\
RO4350B feedthrough & \cite{aprile2011a} & prepreg & 2.70E+01 & 1.80E+01 & 10 & & & & \\
BeCu D-sub pins * & \cite{aprile2017a} & per-pair, 0.33g & 7.90E-07 & 2.60E-07 & 7.50E-06 & 6.61E-03 & & & 4.00E-02 \\
fischer connector * & ILIAS & per piece, 20 48 458 & 9.00E-03 & 2.00E-03 & & & & & 2.30E-02 \\
resistor * ** & & per piece & 5.00E-06 & 5.00E-06 & 5.00E-06 & & & & \\
alumina & ILIAS & UKDM\#8 alumina gel & 4.938271605 & 0.065853659 & 0.588235294 & & & & \\
    \hline
    \end{tabular}
\end{sidewaystable}

\end{comment}


\begin{comment}
\begin{table}[ht!]
    \centering
    \caption{Typical materials found within a dilution refrigerator used for superconducting qubit operation. Not all possible materials are shown. A focus is given to materials either close to the qubit, having high relative levels of trace radioactive concentrations, or that have substantial mass. \JLO{Ben check:}{In this work, these approximate masses and number are used to normalize the simulated rate and dose per disintegration determined using \geant{}}. The assay column refers to the categories presented in Table~\ref{tab:radiopurity_lvls}. Location column gives the approximate placement within a dilution refrigerator; \JLO{Drop? $\rightarrow$}{exact locations within the radiation transport simulation model are not reported}. Cold stage abbreviations: Exp. = Experiment, MC = Mixing Chamber, CP = Cold Plate, ST = Still. \JLO{Fix: }{Items noted with an asterisk, *, are\ldots}. \BML{BML:}{I propose we drop this table. The only info not in table 8 is which ``hit efficiency'' location we pegged each row to, which we could include in Table 8 if we really wanted to}}
    \label{tab:radiopurity_lvls_inst}
    \begin{tabular}{lrrll}
    \toprule
Component & Mass (\JLO{}{UNIT}) & Number & Assay & Location \\
\midrule
Interposer RO4350B & 0.001 & 1 & RO4350B feedthrough & Interposer board \\
Interposer alumina & 0.001 & 1 & alumina & Interposer board \\
Interposer kapton & 0.001 & 1 & kapton & Interposer board \\
Chip wirebonds & 1.0E-6 & 10 & Al-Si bonding wire & Interposer board \\
Package wirebonds & 1.0E-5 & 10 & gold & Interposer board \\
Package fasteners & 3.0E-4 & 10 & brass & Package \\
Package & 0.1 & 1 & copper & Package \\
Package coax connectors & 1* & 10 & mmcx & Package \\
Coax cable near package & 0.1* & 10 & RG174 & Exp. stage \\
Exp. stage & 2 & 1 & copper & Exp. stage \\
Shield copper & 1 & 1 & copper & Exp. shield \\
Shield aluminum & 1 & 1 & aluminum & Exp. shield \\
Shield cryoperm & 1 & 1 & mumetal & Exp. shield \\
MXC RF feedthroughs & 1* & 20 & mmcx & MC Stage \\
MXC DC feedthroughts & 1* & 2 & fischer connector & MC Stage \\
RF circuitry & 1* & 10 & resistor & MC Stage \\
MC Stage & 4 & 1 & copper & MC Stage \\
CP Stage & 3 & 1 & copper & CP Stage \\
ST Stage & 6 & 1 & copper & ST Stage \\
4K Stage & 9 & 1 & copper & 4K Stage \\
50K Stage & 5 & 1 & copper & 50K Stage \\
Vacuum Flange & 20 & 1 & steel & Vacuum Flange \\
Upper Vacuum Can & 8.5 & 1 & aluminum & Upper Vacuum Can \\
Lower Vacuum Can & 14 & 1 & aluminum & Lower Vacuum Can \\
Upper 50K Can & 2.4 & 1 & aluminum & Upper 50K Can \\
Lower 50K Can & 3.6 & 1 & aluminum & Lower 50K Can \\
4K Can & 4.3 & 1 & aluminum & 4K Can \\
Still Can & 6.8 & 1 & copper & Still Can \\
Gold plating & 0.1 & 1 & gold & Exp. stage \\
Gold plating & 0.1 & 1 & gold & MC Stage \\
Gold plating & 0.1 & 1 & gold & CP Stage \\
Gold plating & 0.1 & 1 & gold & ST Stage \\
    \bottomrule
    \end{tabular}
\end{table}
\end{comment}





\begin{comment}
\begin{table}[h]
\caption{\label{table:} \note{[Simplified table - only includes item. For each item assume standard practice materials.}}
\begin{center}
\begin{tabular}{l | c | c | cccccc}
\multicolumn{3}{c}{} & \multicolumn{5}{c}{Isotope concentration (mBq/kg)} \\
{Item}	&	{Mass (g)}	&	{Proximity}	&	{$^{238}\mathrm{U}$}	&	{$^{232}\mathrm{Th}$}	&	{$^{210}\mathrm{Pb}$}	&	{$^{60}\mathrm{Co}$}	&	{$^{40}\mathrm{K}$}	\\ \hline\hline
Wirebonds	&	1 $\mu$g	&	$<$ 1 mm	&	---	&	---	&	---	&	---	&	---	\\ Adhesive	&	$<$1 mg	&	$<$ 1 mm	&	---	&	---	&	---	&	---	&	---	\\
Interposer	&	10 g	&	1 mm	&	---	&	---	&	---	&	---	&	---	\\
Device Package	&	100 g	&	1 cm	&	---	&	---	&	---	&	---	&	---	\\
Connectors	&	10 g	&	1 cm	&	---	&	---	&	---	&	---	&	---	\\
Coaxial cables	&	10 g	&	10 cm	&	---	&	---	&	---	&	---	&	---	\\
Shielding	&	3 kg	&	10 cm	&	---	&	---	&	---	&	---	&	---	\\
\end{tabular}
\end{center}
\end{table}
\end{comment}


\begin{comment}
\begin{table}
    \centering
    \caption{List of typical instrumentation materials found within a dilution refrigerator used for superconducting qubit operation. Not all materials are shown; focus is given to those materials either close to the qubit or having high relative levels of trace radioactive concentrations. The approximate massed and radio-contaminant levels are used to normalize the simulated dose per disintegration using \geant{}. \JLO{}{PNNL will in fill the radiopurity numbers (and then run the simulations).} }
    \label{tab:radiopurity_lvls_inst}
    \begin{tabular}{lllc||cccccc}
    \multicolumn{4}{c||}{Instrumentation materials} & \multicolumn{6}{c}{Isotope concentrations (mBq/kg)} \\
    Item & Material & Prox. & Mass & $^{238}$U & $^{232}$Th & $^{210}$Pb & $^{60}$Co & $^{40}$K & Ref. \\ \hline \hline
    \multicolumn{3}{l}{Device package} & & & & & & & \\
    \quad Wirebonds & Al-Si & mm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Interposer & TMM10 or Alumina & mm  & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Housing screws & Brass & mm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Housing & OFHC Cu & cm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Solenoid bobbin & NbTi & cm  & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Connectors & Ceramic & cm  & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Connectors & CuTe & cm  & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Housing screws & Brass & cm  & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    RF coaxial cables & Sn/Cu, PTFE, Ag coated Cu & cm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    \multicolumn{3}{l}{E\&M \& IR shielding} & & & & & & & \\
    \quad Cu-shield & OFHC (painted black) & cm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Al-shield & Al 6061 & cm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Cryoperm & Ni, Fe, Mo & cm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    \multicolumn{10}{l}{\textbf{\JLO{}{TEMPTED TO LEAVE OUT EVERYTHING BELOW HERE}}} \\
    \hline
    \multicolumn{3}{l}{Microwave components} & & & & & & & \\
    \multicolumn{2}{l}{\quad Minicircuit VLFX} & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \multicolumn{2}{l}{\quad K\&L LPF 12~GHz} & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \multicolumn{2}{l}{\quad RLC Electronics} & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \multicolumn{2}{l}{\quad RF Choke/Diplexer} & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    Circulators/Isolators & Ferrite, Cryoperm & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    Switches (radial) & Stainless steel & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    \multicolumn{3}{l}{DC wiring} & & & & & & & \\
    \quad Micro Dsub & Stainless Steel & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Thermalization bobbin & OFHC?, Au plated, Epoxy dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad DC filters & & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    Superconducting coax & NbTi, PTFE & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    \multicolumn{3}{l}{Thermometry} & & & & & & & \\
    \quad RuOx & RuOx & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad Heater (MXC) & & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \quad PT1000 & & dm & & -- & -- & -- & -- & -- & \cite{CITE} \\
    \hline
    \hline
    \end{tabular}
\end{table}
\end{comment}

%%%
\subsection{Ionizing radiation contributions by source}

As noted in the cosmogenic and terrestrial background evaluations in prior sections, the estimated ionizing radiation event rate within the qubits is anticipated to be on the order of $10^{-3}$\si{/s/g} and the average radiation dose (power) to be on the order of \SI{1}{keV/s/g}. 
%This factor is expected to dominate the ionizing radiation dose exposure of the qubits. 
The decay of known radio-contaminants uniformly distributed within components of the dilution refrigerator were simulated using \geant{} to estimate the energy spectrum of the absorbed dose for each isotope. The associated energy deposition spectrum was then normalized to reported contamination levels provided in Table~\ref{tab:radiopurity_lvls}. For each of the components listed in Table~\ref{tab:internalrate}, we simulate decays of each isotope uniformly throughout a representative volume for that component, record the counts and energy deposited in the qubit chips, and normalize by the assumed mass and contamination level. Section~\ref{sec:append-hiteff} provides more detail on the calculation for each contribution. 

The estimated rate and dose from internal sources is reported in Table~\ref{tab:internalrate}. Two features are worth exploration. First, ceramic PCB interposers generate enough dose in the device substrate to almost negate the radiation shield. Clearly, alternatives must be identified for any radiation-sensitive device. Second, the total estimated rate from internal sources including the shield is approximately twice the residual rate from external gammas with the shield in place. This indicates that further increasing the lead shield efficiency from the design presented in this work will have limited effect unless internal sources are reduced first. Since a handful of sources (coax connectors, aluminum shield and vacuum can) dominate the internal budget, signficant headway can be made relatively straightforwardly, as described in more detail in the next section. 

%\textbf{Edit and update this paragraph after more instrumentation materials are simulated:}A more detailed study of the internal sources would be required. However, the largest single contributor to the induced rate is the device packages (the small copper boxes that house 9 silicon chips in the simulated geometry). This is unsurprising as that is the material closest to the qubit chips. This suggests that further reducing the internal rate could be attained by replacing the device packages with higher-purity copper screened for radioactive contamination, and possible deploying additional shielding inside the fridge. 

%The approach used in this evaluation was to model as many isotopes as possible in the copper mount plate directly adjacent the the qubit array to determine which nuclides produced appreciable tallies. The total energy deposited was tallied per primary and the sum of all energy deposited divided by the number of primaries was considered the mean energy deposited per disintegration. This mean energy per disintegration was multiplied by the total mass of the corresponding object, the mount plate in this case, and disintegration rate per kilogram to estimate the energy deposition per second. Isotopes that did not produce appreciable energy deposition tallies over 1e7 primaries were assumed to be inconsequential as it was not expected that primary or secondary gamma or x-ray emissions generated from charged particle decay would pierce the copper or bronze radiation shield effectively modeled as the mounting plate.

%As an example calculation, the energy deposition spectrum shown in figure \ref{fig:co60_kerma_spectrum} was tallied over $10^7$ primaries simulated; this spectrum has a mean energy 0.169~MeV and a total of 12,040 counted tallies i.e. there is a total of 0.169~MeV$\cdot$12,040~tallies/1E+7~primaries=2.03E-4~MeV$\cdot$tallies/primary. In this sense tallies per primary is equivalent to depositions per decay when transitioning to a reference of 0.2~mBq/kg or decays/sec/kg. Multiplying the model estimated MeV$\cdot$depositions/decay by the reference activity gives 4E-6~MeV$\cdot$depositions/sec/kg. The OFHC mounting plate is 18~cm on a side and 0.635~cm thick with a density of 8.96~g/cc. Using the plate dimensions and mass, the energy deposition per second is (18$\cdot$18$\cdot$0.635)cc$\cdot$8.96~g/cc$\cdot$kg/1000g$\cdot$4E-6~MeV$\cdot$ depositions/sec/kg=7.5E-5~MeV$\cdot$deposition/sec.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.7\textwidth]{figures/co60_mount-plate_qubit_kerma.pdf}
%    \caption{Kerma deposition profile in the qubit array from $^{60}$Co contamination in the rear OFHC %mount-plate of the dilution refrigerator per decay.}
%    \label{fig:co60_kerma_spectrum}
%\end{figure}

%\begin{table}[ht]
%    \centering
%    \begin{tabular}{c|cccccccccccc}
%        Contaminant (MeV/sec)  & OFHC      & 316S      & In     \\ \hline
%        $^{238}$U              &           &           &        \\
%        $^{235}$U              &           &           &        \\
%        $^{234}$Th             &           &           &        \\
%        $^{232}$Th             &           &           &        \\
%        $^{228}$Ac             &           &           &        \\
%        $^{214}$Bi             & 4.25E-7   &           &        \\
%        $^{214}$Pb             & 5.89E-8   &           &        \\
%        $^{212}$Pb             & 2.42E-8   &           &        \\
%        $^{210}$Pb             &           &           &        \\
%        $^{208}$Tl             & 2.36E-7   &           &        \\
%        $^{137}$Cs             & 1.72E-8   &           &        \\
%        $^{60}$Co              & 7.50E-8   &           &        \\
%        $^{40}$K               & 8.75E-8   &           &        \\ \hline
%        Total                  &           &           &
%    \end{tabular}
%    \caption{Radio-contaminant levels used to normalize the simulated kerma dose per disintegration estimated using GEANT4.}
%    \label{tab:radiopurity_lvls}
%\end{table}

%Monte Carlo methods are, inherently, computationally and time intensive; so much so that obtaining statistically relevant results with singular compute nodes within days to weeks is challenging. This complication has been encountered in other cosmic background simulations; thus, highlighting the need to accelerate the simulation process. Variance reduction is the most common method of mitigating this problem.

%Two methods of variance reduction were explored: 1) proposed by Battistoni in \citep{battistoni_monte_1997} which makes use of repeated geometries to increase the tally count-rate, and 2) source biasing. Figure \ref{fig:underground} depicts the model configuration of a dilution fridge housing sensitive instruments within a concrete shell and 19~m soil overburden.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\textwidth]{figures/underground_model.png}
%    \caption{CAD rendering of dilution fridge within a concrete cavity beneath a 19~m %overburden.}
%    \label{fig:underground}
%\end{figure}




%%%
%%% Discussion
%%%

\section{Discussion}\label{sec:discussion}

\subsection{Performance of superconducting devices in this design}
The combination of overburden and lead shielding described in this work should reduce the total ionizing radiation interaction rate for devices inside the dilution refrigerator by approximately 95\% compared to an unshielded system operating at sea level.\footnote{This calculation is based on the measured vertical muon flux reduction of 85\%. Since the muon flux at higher angles and the fluxes of other cosmic ray secondaries (primarily neutrons, protons, and gammas) are more strongly attenuated, this figure should be conservative.} Here we assume some care is taken to avoid introducing items with high radioactivity into the fridge such as ceramic PCBs. The primary purpose of this design is to be able to study superconducting devices in a controlled radiation environment. % For sufficiently advanced devices, we also might expect to see an immediate improvement in superconducting qubit performance, namely decreases in the rates of both single-qubit decoherence and correlated decoherence errors. The forthcoming projections are, of course, under an assumption that no other deleterious effects are present in the environment of the superconducting qubits. Said another way, all the following comparisons only apply under conditions such that, ``If the only detrimental environmental effect at play is ionizing radiation, then the shallow underground, shield system would provide\ldots''

A controlled radiation environment enables testing of superconducting qubits and quasiparticle sensitive detectors for the effects of ionizing radiation. The simplest use case of the design includes a/b comparison of device performance between an above-ground laboratory and the shallow underground laboratory. Based on the experiment by Veps{\"a}l{\"a}inen et.\ al.~\cite{vepsalainen2020}, we expect a $\sim$2.4-fold decrease in the radiation-induced decoherence rate to $\Gamma_1\sim1/(\SI{10}{ms})$ based on our radiation dose (\SI{7.5}{keV/g/s}). Despite the significant reduction of background radiation in our design, we expect only a minute effect on the actual coherence time of superconducting qubits as characterized using typical inversion recovery measurements which average many, $\mathcal{O}(10^3)$, rounds of state preparation and measurement over $\mathcal{O}(\mathrm{min})$ timescales. 

% For the device studied by Veps{\"a}l{\"a}inen et.\ al.~\cite{vepsalainen2020}, the authors estimated the rate of bit-flip errors induced by ionizing radiation to be $\Gamma_1\sim1/(\SI{4}{ms})$ driven by an external radiation power of \SI{43}{keV/g/s}. In their model, the ionizing radiation-induced error rate is directly proportional to the steady-state non-equilibrium quasiparticle density, which in turn is proportional to the square root of the incoming radiation power. Thus, a similar device operated in the underground shielded dilution refrigerator we describe (\SI{7.5}{keV/g/s}) would see a $\sim$2.4-fold decrease in radiation-induced decoherence rate to $\Gamma_1\sim1/(\SI{10}{ms})$. We, however, suspect the interaction \emph{rate} is a better model as the ionizing event rates decreases, as is the goal of the system design presented in this report.

%If instead the ionizing radiation-induced errors arise from the prompt response of ionizing radiation interactions rather than a steady-state excitation, the decoherence rate would be directly proportional to the interaction rate and thus would reduce to $\Gamma_1\sim1/(\SI{20}{ms})$ (this is ratio of dose, not ratio of count rate
%\BML{}{Is there a ``threshold'' error rate that this number might be relevant to?} \JLO{}{Yes, but it will be ``wrong'' as soon as we write it down.}

For example, McEwen et.\ al.\ report ``bursts'' of decoherence errors in multiple qubits on the same chip with short time correlations at an average rate of $\lambda\sim1/(\SI{10}{s})$~\cite{mcewen2022}.  If the error burst rate is directly proportional to the average ionizing radiation interaction rate, such a device in our shielded underground system would observe a burst rate of $\lambda\sim1/(\SI{200}{s})$, assuming the radiation environment in their laboratory is similar to ours when unshielded\footnote{Although an entirely qualitative observation, our experience has shown that buildings vary by ``only'' about a factor 2 in their primordial radiation emission, depending on the materials use in construction.}. For this analysis we have ignored any energy dependence of the event rate. That is, we assume any ionizing radiation event that deposits energy over \SI{3}{eV} threshold is equally likely to produce an error burst. This assumption is supported by observations of SuperCDMS detectors where sub-keV energy deposits excite sensors spread over centimeters of kg-scale devices~\cite{agnese2016}\footnote{Note that SuperCDMS detectors have a substantially different aspect ratio ($\sim$1:3 vs.\ $\sim$1:100 for a typical chip) and are intentionally thermally isolated, both of which features may lead to a more uniform phonon cloud.}. 

%The presence of the gamma shield ``stiffens'' the spectrum, increasing the average energy deposited per interaction.  If error correlations depend on the deposited energy (since higher energy deposited will produce more athermal phonons and quasipaticles), error burst suppression will be less effective. In particular, if the error bursts are driven by cosmic rays, as the McEwen et.\ al.\ authors suggest, the error burst reduction factor would be only 0.15, the attenuation of cosmic ray muons by the SUL overburden, resulting in a correlated error rate of approximately one every 60 seconds. \JLO{JLO:}{I think this last paragraph is confusing. Try the following instead. --- Also, the ``stiffening'' is a red-hearing, in my opinion. Yes, the spectrum gets more energetic on average, but the overall rate drops ``more''. From my perspective, unless the rate is fixed, ``spectrum stiffening'' is a deceptive observation. You could say, ``Big bangs happen on average, but much less frequently.'' Kind of like the evolution of meteor impacts on Earth over time. I much prefer living now (low rate, but with worse consequences\ldots very infrequently).}

We note the title of the McEwen et.\ al.\ report suggestively attributes the observed error bursts to cosmic rays, though the authors do make clear that gamma-rays from naturally occurring radioactivity in the environment can also contribute. Determining the relative influence of cosmic ray secondary interactions and interactions for gamma-radiation is one of the goals of the shallow underground, shielded system. The experimental test is apparent if one hypotheses \emph{only} cosmic rays cause large, correlated error bursts. Under such an hypothesis the error burst improvement that would be observed in the shallow underground lab system would be directly rated to the inverse of the cosmic ray attention factor of 0.15, the attenuation of cosmic ray muons by the SUL overburden. This would result in an estimated correlated error rate of approximately one every 60 seconds. This is in contrast to the average \SI{200}{s} burst rate estimated above. These are clear and distinctive predictions the system presented in this report will test.

Astute readers will notice the three orders of magnitude difference between radiation-driven single-qubit decoherence rates ($1/(\SI{4}{ms})$~\cite{vepsalainen2020}) and correlated catastrophic error bursts ($1/(\SI{10}{s})$~\cite{mcewen2022}) (both assuming an unshielded system at surface). The ``square-root of dose'' scaling assumed for single-qubit error rates was observed when the qubits were exposed to a radiation source $10^4$ times greater than ambient levels~\cite{vepsalainen2020}. The scaling is based on a steady-state excess quasiparticle population produced by incoming radiation power and reduced by quasiparticle recombination. Such a model can only hold where the average time between excitations is comparable to (or shorter than) the recovery time. As the average time between excitations (from all sources, not just ionizing radiation) increases to much longer than the recovery time, one would expect a ``phase change'' to occur, where the steady-state excitation disappears and the single-qubit decoherence rate is driven directly by the stochastic interaction rate. In this limit, the single-qubit decoherence rate would scale proportionally with the correlated error burst rate. Furthermore, the rates would be identical if there is no energy dependence to either. 

Measurements of the recovery time vary considerably: \SI{140}{\micro s}~\cite{wilen2021} and \SI{25}{ms}~\cite{mcewen2022} for qubit error bursts, $\sim$\SI{250}{ms} for kinetic inductance sensors~\cite{cardani2021}\footnote{The authors do not report the recovery time; this estimate is based on analyzing Figure 1 of Ref~\cite{cardani2021}.}.  These values suggest that the ionizing radiation contribution to the steady-state quasiparticle population should already be negligible at typical ambient levels of radioactivity and certainly so in an underground, shielded system. This is somewhat at odds with the observation that an inefficient gamma shield (which removed less than half of the ambient ionizing radiation) produced a measurable decrease in decoherence rate~\cite{vepsalainen2020}. However, if the excitation has a second, independent component with much longer recovery time (e.g., slow release of charge trapped in shallow crystal defects~\cite{shockley1952}), this would not have been observed in any of the cited measurements and steady-state behavior may remain relevant, though it may have some dependence other than square-root. The purpose of this digression is to emphasize the overly simplified nature of the extrapolations presented above.

\subsection{Further reduction of ionizing radiation interactions}
Assuming the extrapolations in the preceding section are valid, the modest depth and shield we describe in this work is sufficient to reduce correlated qubit error rates to negligible levels. Use of a classical co-sensor to identify and reject calculations where an error burst occurred would further prevent erroneous trials from contaminating a result set~\cite{orrell2021}. Thus, devices operated in this shield would generate only stochastic, uncorrelated errors well described by conventional quantum error correction.  

Nevertheless, in this section we examine what steps would be required to further reduce ionizing radiation if so desired. For each successive reduction step, we target and mitigate the highest remaining source. Eventually we reach the ultimate background limits achieved by advanced fundamental physics detectors searching for interactions with galactic dark matter. 

\paragraph{Radiopurity of packaging and instrumentation}
The most signficant sources of ionizing radiation in a device are high in radioactive contamination and either very close to the device or very massive. By far the most signifcant source of radiation under the researcher's control is the PCB interposer to which superconducting devices are often attached, which are frequently made of ceramic materials with high levels of radioactivity. As Table~\ref{tab:radiopurity_lvls}, the radiation interaction rate from one gram of such materials would dominate the total radiation budget in our shielded system and is in fact comparable to the total unshielded rate. Low background detectors often use polyimides (Kapton and cirlex), silicon, or sometimes sapphire for similar purposes.  Kapton, for example, would produce a radiation interaction rate roughly 100 times lower than alumina, but is likely unsuitable due to the high dielectric loss at typical superconducting qubit frequencies. 

Likewise, RF coax connectors on the device package generate high rates due to their close proximity and relatively high radioactivity (usually from BeCu and sometimes also ceramic insulator, though the latter is uncommon for SMA connectors). The coax cables themselves are much lower radioactivity than the connectors, and connectors $\sim$\SI{10}{cm} away at the MXC stage contribute significantly less, so only the connectors on the device package would need to be replaced. 

\paragraph{Cosmic Ray Muons}
If no ceramic interposer is used, cosmic ray muons are the dominant source of ionizing radiation in devices operating in the underground shielded system. Further reduction would require a deeper site. A further reduction factor of 1000, at which point the muon rate is below the rate from the fridge itself, would require a depth of roughly  \SI{1}{kilometer} water equivalent~\cite{laubenstein2004}.

Depending on device and use case, an alternative to operating at a deeper site may be to employ a muon veto system as is commonly done for sensitive radiation detectors~\cite{knoll2010}. A muon veto would detect whenever a muon passed through some ``shell'' surrounding the device of interest, allowing for the rejection of any data generated during that time. A veto system would not prevent errors in a superconducting qubit, but could provide a source to apply quantum fault mitigation~\cite{orrell2021}. 

\paragraph{Improved low background shielding}
After cosmic rays, the next most siginficant source of events are residual environmental gamma rays and emissions from the shield itself. Further reducing the ambient gamma flux is not as straightforward as increasing the shield thickness. As Table~\ref{tab:ratevsshieldthick} shows, the effect of the open top of the shield that allows free access to the vacuum flange is a significant source of the residual flux. Closing all of those openings would require a substantially more complex shield design.  Eventually, small gaps between lead bricks would become significant, requiring multiple layers to be staggered or redesigned with curved or ``chevron'' interfaces. 

Reducing the contribution from the shield itself is straightforward but costly. The most significant source is \iso{Pb}{210} present at high levels in all recently-manufactured lead. To reduce this source, the innermost several centimeters would have to be replaced with so-called ``ancient lead,'' often obtained from ancient shipwrecks~\cite{knoll2010}. The aluminum plates that hold the fridge and lead that are inside the shield also produce significant rates of radiation interactions. (Note that aluminum and steel plates and structural framing outside the shield is not included as it is assumed to be insignificant compared to the total environmental gamma flux.) These would need to be removed from the design or, if not possible, replaced with a lower background material such as OFHC copper. 

\paragraph{Radiation from the dilution refrigerator}
Further reducing the ionizing radiation event rate would require modifying the dilution refrigerator itself. The majority of the rate comes from the vacuum and IR cans, which could all be replaced with copper. Any further reduction would require completely rebuilding every part of the setup including the dilution refrigerator with ultra low-background materials and techniques similar to a dark matter experiment. As an example, wirebonds may become a relevant source at this level. Thus the ``practical'' limit is a reduction factor of $10^{-4}$ to $10^{-5}$.  Following our analysis above, this would result in ionizing radiation-limiting $T_1$ times for the Veps{\"a}l{\"a}inen et.\ al.\ device of $\sim\SI{1}{s}$ and error burst rates for the McEwen et.\ al.\ device below 1 per day, again with the large caveat of assuming that \emph{only} ionizing radiation matters to device performance.

As a partial alternative to complete redesign, an internal radiation shield may reduce the ionizing radiation backgrounds from the dilution refrigerator. In a prior unpublished study, we estimate that a \SI{5}{cm} thick tungsten shield placed around the qubit package, with slits to allow cable connections, would attenuate the environmental gamma flux by a factor of $\sim$50; a similar reduction factor is expected for the residual flux after the steps above have been implemented. The addition of so much mass to the mixing chamber stage would dramatically increase cooldown times. We also did not consider any intrinsic radioactivity of the tungsten itself in this estimate. We chose tungsten over lead due to its higher gamma attenuation coefficient per unit thickness than lead, but an ancient lead inner shield would have similar performance while being considerably less massive and easier to machine. 

\paragraph{Ultimate limits}
The next generation of dark matter detectors expect to attain sufficient shielding and background reduction efficiency that they will be limited by \iso{Si}{32} in the silicon substrate~\cite{PhysRevD.95.082002, ORRELL20189, aguilar-arevalo2022}. \iso{Si}{32} has been measured in silicon CCDs to be approximately {10--100 /kg/day}~\cite{Aguilar-Arevalo2015, Aguilar-Arevalo2021}, or a reduction factor of $\sim$$10^{-6}$ to $10^{-7}$ compared to unshielded surface operation. Attaining these levels of backgrounds requires tens of millions of dollars for shielding and custom ultra low-background components. These experiments operate in dedicated underground laboratories at depths of several kilometers water equivalent to obtain the necessary reduction in cosmic ray muon fluence~\cite{mei2006}.


==> oldstuff/discussion_original.tex <==

The natural questions to raise regarding this design are:
\begin{itemize}
    \item How much improvement will the shielded system provide?
    \item How does this design compare to existing shielded systems?
\end{itemize}
These are in fact the open research questions being pursued.

The first question is implicitly framed with respect to the performance of any superconducting qubit operated above ground, outside of a lead shield, in comparison to operation in the underground, shielded system described in this report. The metric for comparison is most reasonably the qubit coherence time. The second question is needed to help answer the first, but can also be inferred to ask for a comparison to ``the best possible'' (deep) underground, ionizing radiation shielded systems ever built. The follow subsections evaluate these questions with one substantial caveat: At the time of this report, ionizing radiation is emphatically \emph{not} the dominant decoherence mechanism for superconducting qubits. Thus, all conclusions we will draw must be prefaced with, ``If no other decoherence mechanisms were present, then the decoherence due to ionizing radiation would\ldots''.

%%%
\subsection{Reduction of ionizing radiation external power}\label{sec:powerdose}
In a recent report~\cite{vepsalainen2020}, the ambient external power attributed to ionizing radiation was $P_{\mathrm{ext}} = 0.10$~keV~mm$^{-3}$~s$^{-1}$. Approximately 60\% was attributed to naturally occurring gamma-ray radiation and the remaining 40\% was attributed to cosmic rays. To convert the external power into the units used in this report, we divide by the density of silicon, $\rho_{\mathrm{Si}}=2.33$~g$\cdot$cm$^{-3}=0.00233$~g$\cdot$mm$^{-3}$, arriving at $P_{\mathrm{ext}} = 42.9$~keV/s/g. This value is comparable\footnote{PMH: The $P_{ext}$ value includes gammas and above-ground muons. To make a fair comparison to Table 3, the muon contribution should be removed $P_{ext, gamma}$ = 0.06 keV/mm3/s = 25.8 keV/s/g, which is actually 0.5 the dose rate simulated for gammas in the SUL. JLO: This is totally within my sense of ``comparable''. I'm inclined \emph{not} to provide more detail since that gives an incorrect sense of how precise these estimates can be, given the current state of the art.} to the estimate provided in Tab.~\ref{tab:ratevsshieldthick} for an un-shielded system exposed to gamma-rays from the concrete laboratory walls, having a dose rate of $53.6$~keV/s/g.

The shield design presented in this report improves\footnote{PMH: Now this is a comparison between the MIT gammas unshielded and the SUL gammas shielded? This doesn't seem to be a fair comparison without resolving the discrepancy between the laboratory gammas of MIT and SUL. JLO: I'll look at these numbers again.} on the gamma-ray dose rate by a factor of $\sim$450 (\textit{i.e.}, gamma does rate of $0.12$~keV/s/g). However, the residual cosmic rays in the SUL are the dominant dose rate which shown in Tab.~\ref{tab:ratevsshieldthick} to be $1.65$~keV/s/g, a factor of 26 improvement on the external power inferred in Ref.~\cite{vepsalainen2020}. Ref.~\cite{vepsalainen2020} makes a suggestion that if no other decoherence mechanisms were present, then the decoherence due to ionizing radiation in their system would permit superconducting qubits to operate with coherence times in the range of approximately 3,130~$\mu$s to 3,950~$\mu$s. Using the same method of extrapolation, we would therefore estimate the residual cosmic ray dose rate in the shielded system described in this report would permit superconducting qubits to operate with coherence times in the range of approximately 17,000~$\mu$s\footnote{PMH: Note that this is calculated using the sqrt of dose. JLO: Check ``math'' and perhaps add textual note.}, once again assuming no other decoherence mechanisms were present.

This evaluation is at best approximate. Furthermore, note the above approximation relies on a comparison between external power, or does rate, within the context of the model of Ref.~\cite{vepsalainen2020}. We believe this is the reliable predictor of performance for an assumed ``uniform'' ionizing radiation field impinging on the superconducting qubits. The next section, however, provides a distinct contrast when a comparison based on interactions rates is performed.

%%%
\subsection{Reduction of catastrophic error bursts}\label{sec:cosmicrate}

PMH\footnote{We can use the McEwen, et al. result to estimate an ``interaction limited'' average coherent time. When an event occurred they measured an average qubit coherence, 1/T1 = 1/(730 ns). Events occurred at a rate 1/(10 s). The duration of each event is 15 ms. We calculate the average T1 limit due to these events as, 1/T1avg = (15 ms/10 s)*(1/(730 ns)) = 1/(500 us). Additionally, to compare to the MIT experiment, we scale this 1/T1avg by chip size to get, 1/T1avg (MIT) = 1/(5 ms), which is consistent with the MIT experiment.}

In a recent report~\cite{mcewen2021}, catastrophic error bursts in a multi-qubit superconducting device were attributed to cosmic rays directly striking the device\footnote{PMH: the conclusions from McEwen, et al. actually attribute a larger portion of events to gammas than to cosmic ray muons (see SM). They report expected interaction rates based on the calculation in Wilen, et al. by simply scaling by the chip geometry. Also note that the muon interaction rate calculation in Wilen, et al. quite possibly incorrect (a gross underestimate). JLO: OK. I need to go back and reread.}. The report showed the mean frequency of cosmic ray strikes was roughly once every 10~s. In this report we have suggested that cosmic muon ray interactions will drive the ionizing radiation disturbances of superconducting qubits in the underground shielded system we describe. Thus, we can make a direct comparison to the cosmic ray rate estimated shown in Tab.~\ref{tab:ratevsshieldthick} of $5.07\times10^{-3}$~counts/s/g.

The Google Sycamore processor silicon chip is 10~mm $\times$ 10~mm $\times$ 500~$\mu$m and resides on a carrier chip (20~mm by 24~mm), connected by 5~$\mu$m indium bump bonds (all dimensions from Ref.~\cite{mcewen2021}). For simplicity we assume the indium bump bonds provide thermal separation due to the large In superconducting gap (\JLO{}{Does this even make sense?}). Thus, the chip target is 0.1165~g of silicon. This converts the one cosmic ray strike every tens seconds to a rate of approximately 0.86~counts/s/g in the units of this report. Comparing the hit rate on the Google Sycamore to that expected in the shielded SUL system (5.07 $\times$ 10$^{-3}$~counts/s/g)\footnote{PMH: The comparison should be made to the total SUL interaction rate (gammas $+$ muons). JLO: Yes, I do need to make this adjustment, for sure.}, we would therefore infer a reduction in the catastrophic error burst rate by a factor of roughly 170. Thus, in the shielded SUL system, the frequency is on average one cosmic ray every 1700~s ($\sim$28~min). We note in passing if cosmic rays are ignored, the same comparison suggests that on average one gamma-ray interaction will occur approximately every 3.2~hours.

Caveats for this analysis: SCDMS 1~kg shows phonons easily populate sensors. Gram-based and orientation matters, so this is to be considered.

%%%
\subsection{Comparison with deep underground systems}\label{sub:ugcomparison}

\textbf{I want to add a comparison to SuperCDMS and DAMIC, as best we can. I would like to also touch on the rate expected due to Si-32.}

\paragraph{Si-32 and solar neutrinos - John - Remove this paragraph heading}
As an ultimate limiting case, it is expected trace levels of \iso{Si}{32} are present in the silicon chip substrate~\cite{ORRELL20189}. It is not readily feasible to directly measure the \iso{Si}{32} levels in the chip. However, it is expected the concentration is such that there is on order of 10-100~decays/(kg d)~\cite{Aguilar-Arevalo2015, Aguilar-Arevalo2021}, in single chip of approximately 15~mg. As will be shown, the rate of \iso{Si}{32} decay events is orders of magnitude below the rate of cosmic ray and gamma ray interactions anticipated for the shallow underground system described in this report. Nevertheless, the expected intrinsic level of \iso{Si}{32} present in the silicon will serve as an effective point of comparison to current state-of-the-art, research-grade, deep underground, ultra-low radioactivity background science experiments.

``These detectors consist of cylindrical crystals, 100 mm in diameter and 33.3 mm thick. Each Ge(Si) crystal has a mass of 1.39(0.61) kg.''\cite{PhysRevD.95.082002}

\begin{table}
    \centering
    \caption{ULB comparison table. Calculate and check all numbers! Explanation should be in text body. (Ave. 1-50 keV in 100~mm dia. $\times$ 33.3~mm thick Si)}
    \label{tab:ulbcomparison}
    \begin{tabular}{lllc}
     \multicolumn{2}{l}{Source}    & (Unit) & Ref. \\
                  & Configuration & Value & \\
      \hline \hline
      \multicolumn{2}{l}{Cosmic rays}  & (\#/cm$^2$/min) & \\
                   & Surface & 1.00E+00 & \\
                  & PNNL SUL & 1.67E-02 & \\
                   & LGNS     &   1.67E-05 & \\
                   & SNOLAB  & 2.26E-07 & \\
       \hline
       \multicolumn{2}{l}{Gamma rays} & (\#/g/min) & \\
                  & Laboratory  & a lot & This work \\
	& Inside PNNL SUL Shield & 1/500 of lab & This work \\
	& SuperCDMS & $9.6\times10^{-6}$ & ``15+0.07+88 iZIP'' \cite{PhysRevD.95.082002} \\
	\hline
	\multicolumn{2}{l}{Intrinsic \& neutrino} & (\#/g/min) & \\
        & Si-32 & $2.4\times10^{-5}$ & ``260 iZIP'' \cite{PhysRevD.95.082002} \\
        & Solar neutrinos (elastic) & $1.5\times10^{-10}$ & ``1600 iZIP'' \cite{PhysRevD.95.082002} \\
    \hline
    \end{tabular}
\end{table}


%%%
\subsection{Other speculations (now removed) \JLO{}{``Done''}}\label{sub:speculations}

\JLO{Note:}{I have removed two sub-sections. One sub-section basically just summarized the above two subsections, while reminding the reader ``Ionizing radiation is \emph{not} the current problem''. The other sub-section made some speculative comments related to adding \emph{active} veto systems to the shield. A perceptive reader will realize that our shield design is \emph{entirely passive} while most all modern system have active cosmic ray vetos. Sure, we want to explore that, but speculating on that detail seems far too speculative for this already very speculative ``design'' paper. It seems that ``\textit{Impact of radiation veto systems on superconducting quantum computing devices}'' is really it's own research outcome. So let's wait till we are working on it to write about it.}

%%%
%\subsection{Benefits from underground shielded systems}\label{sub:benefit}
%
%The above subsections present several perspectives on the possible benefits of locating superconducting quantum computing devices in underground, ionizing radiation shielded systems. A few summarizing comments are in order:
%\begin{itemize}
%    \item Current superconducting qubits are \emph{not} limited by ionizing radiation.
%    \item If ionizing radiation \emph{does} become a limiting factor, a shallow underground shielded system like the one described in this report has the potential to provide:
%    \begin{itemize}
%        \item An environment permitting superconducting qubits to operate with up to 17~ms coherence times with minimal disturbances from ionizing radiation.
%        \item A 170-fold reduction in cosmic ray induced catastrophic error bursts in Google Sycamore-like devices.
%    \end{itemize}
%    \item 
%\end{itemize}
%These projections provide the rationale for an investigation of whether these benefits can be achieved. Even if they are not, we believe such systems will provide a testing ground for discovering and exploring a myriad of \emph{non}-ionizing radiation impacts to superconducting coherence. Essentially, the confidence provided that ionizing radiation is not playing a substantial roll in decoherence effects, will likely permit new studies of material and device effects.

%%%
%\subsection{Application to quantum computing systems}\label{sub:ugquantum}
%
%An important consideration regarding the shield thickness is that we have assumed no active vetoing of the cosmic ray muons. Low background counting systems such as HPGe detectors often employ such vetoes (typically large plastic scintillator panels) to reduce cosmic ray-induced backgrounds by at least an order of magnitude. Some types of superconducting sensors may benefit from such a veto, but it is not clear whether qubits or other quantum instruments can. For example, if cosmic ray muons generate prompt quasiparticle bursts~\cite{cardani2021}, this will lead to coincident decoherence in a quantum device. In this case, a muon veto may be able to reject bad data points from some kinds of quantum sensors. Alternatively, it could be that the overall decoherence rate is the important factor, in which case flagging the time of decoherence with the veto may not have any practical benefit. Moreover, if the energy input from cosmic rays leads to an excess steady-state quasiparticle population~\cite{vepsalainen2020}, decoherence might not be coincident with muon events, in which case a muon veto will again not be effective. 
%
%If the cosmic ray muon rate can be lowered, either by operating in a deeper site or by the use of a muon veto, the shield would need to be made thicker to keep the ambient gamma rate below the cosmic rays. However, this may not be as simple as increasing the thickness with the design we have presented. First, as the shield gets thicker, the rate from gammas entering the shield through penetrations without direct line-of-sight to the qubits becomes more important. Additional ``shadow'' shielding may be needed to reduce this effect. Second, internal sources also become relatively more important. At some point, there are no additional gains to be had from a thicker shield unless the radioactivity of all components inside the dilution fridge is controlled first. As Table~\ref{tab:internalrate} shows, we expect the rate from sources of radiation inside the fridge to be roughly half (\textbf{NEEDS UPDATE}) of the residual external rate with the current shield design, so improved shielding will again have limited returns without redesigning the fridge to use low radioactivity components. Finally, there are additional engineering considerations, particularly for the upper shield sections that are held up by the vendor support frame, which might need to be reinforced if significant additional weight is added.
%
%\textbf{Add paragraph on chip-base burst veto, perhaps?}
%
%\textbf{Concluding paragraph on how, until qubits can reach much longer coherent times, shallow shielded DRs without material controls are probably sufficient.}



==> oldstuff/dosetable_original.tex <==
\begin{table}
    \centering
    \caption{Simulated interaction rate and dose from some components inside the dilution refrigerator. The estimated residual rates from cosmic rays in the SUL and external gammas passing through the shield are included for comparison. Likewise, the impact of BeCu pins and \iso{Si}{32} in silicon is shown, but not included in the Total dilution refrigerator (DR) contribution. These last two radiation sources, respectively, bracket the high- and low-levels of ionizing radiation interaction rates achievable in a shielded dilution refrigerator design. Included uncertainties are statistical only. \JLO{}{I recommend removing all the $\pm$ errors; we're doing an order of magnitude assessment.}}
    \label{tab:internalrate}
    \sisetup{separate-uncertainty, table-align-uncertainty=false}
    \begin{tabular}{llS[table-format=2.2]|S[table-format=1.2(1)e-1]|S[table-format=1.2(1)e-1]}
        Component & Material & {Mass} & {Interaction rate} & {Dose rate} \\
        & & {(kg)} & {($10^{-3}$~counts/s/g)} & {(keV/s/g)} \\
        \hline
        Cosmic rays in SUL &  &  & 5.07(5)e0& 1.65(2)e0\\
        \multicolumn{2}{l}{Ambient gammas (shielded)} &  & 7.5(6)e-1 & 1.2(1)e-1 \\
        Shield lead (\iso{Pb}{210}) & Pb & 4870 & & \\
        All DR components &  &  & 4.48(10)e-1& 5.1(2)e-2\\
        All instrumentation  &  &   &                   &                 \\
        \hline
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        \hline
        \multicolumn{5}{l}{Individual contributions to ``All DR components''.} \\
        \hline
        \quad RF cavity & Cu & 2 &1.82(1)e-1 & 2.10(1)e-2 \\
        \quad Vacuum chamber & Al & 22 & 1.13(8)e-1 & 1.3(1)e-2 \\
        \quad 4K can & Al & 3.7 & 5.4(3)e-2 & 5.7(4)e-3 \\
        \quad 4K stage & Al & 8.7 & 7(1)e-3 & 6(2)e-4 \\
        \quad 50K stage & Al & 15 & 7(3)e-3 & 5(2)e-4 \\
        \quad Mixing Chamber (MC) & Cu & 4.6 & 6.7(1)e-3 & 8.6(3)e-4 \\
        \quad 50K can & Al & 6.7 & 5.5(3)e-3 & 7.7(6)e-3 \\
        \quad Still can & Cu & 5.7 & 4.2(1)e-3 & 1.34(8)e-4 \\
        \quad gold plating & Au & 0.2 & 2.53(6)e-3 & 2.2(1)e-4 \\
        \quad Vacuum flange & Steel & 21 & 8(3)e-4 & 7(3)e-5 \\
        \quad Cold Plate & Cu & 3.3 & 6.3(3)e-4 & 1.9(2)e-5 \\
        \quad Still & Cu & 5.9 & 5.0(4)e-4 & 1.6(3)e-5 \\
        \hline
        \multicolumn{5}{l}{\vspace{-0.75em}} \\
        \hline
        \multicolumn{5}{l}{Individual contributions to ``All Instrumentation''. Masses in grams. \textbf{Rows below are notional!}} \\
        \hline
        Wirebonds (4) at each chip & Al-Si &  &  &  \\
        Interposer & Alumina &  &  &  \\
        Housing screws & Brass &  &  &  \\
        Housing & OFHC Cu &  &  &  \\
        Solenoid bobbin & NbTi &  &  &  \\
        Connectors & Ceramic &  &  &  \\
        Connectors & CuTe &  &  &  \\
        RF coaxial cables & Sn/Cu, PTFE &  &  &  \\
        Cu-shield & OFHC Cu &  &  &  \\
        Al-shield & Al 6061 &  &  &  \\
        Cryoperm & Ni, Fe, Mo &  &  &  \\
        Feedthrough at MC & Ceramic/BeCu/? &  &  &  \\
        Feedthrough at LN & Ceramic/BeCu/? &  &  &  \\
        \hline
    \end{tabular}
\end{table}


==> oldstuff/hitefftable_original.tex <==
\begin{table}[ht!]
    \centering
    \caption{Hit efficiency table of discrete ionizing radiation interactions for comparing relative impact of radioactive contaminants in a dilution refrigerator, as modeled by radiation transport Monte Carlo simulations of the design described in this report. Units: counts/gram/second/Becquerel. \BML{BML}:{We should also provide the dose-efficiency table} }
    \label{tab:hiteff}
    \begin{tabular}{l|rrrrrrrr}
    \toprule
%    Source location & \iso{K}{40} & \iso{Th}{232} & \iso{U}{238} & Activation & \iso{Pb}{210} & \iso{Co}{60} & \iso{Cs}{137} \\
%    \hline \hline
%Interposer board & 1.5E+0 & 5.1E+0 & 7.1E+0 & 4.2E-1 & 1.5E+0 & 3.1E-1 & 8.2E-1 \\
%%Packge Inner Surface & 9.8E-1 & 1.8E+1 & 2.0E+1 & 9.5E-1 & 3.8E+0 & 7.8E-1 & 1.1E+0 \\
%Package & 1.3E-2 & 5.9E-2 & 7.3E-2 & 1.4E-2 & 6.8E-3 & 2.1E-2 & 9.5E-3 \\
%%Package Outer Surface & 1.1E-3 & 6.4E-3 & 6.0E-3 & 6.8E-3 & 9.0E-5 & 1.1E-2 & 3.6E-3 \\
%Experiment stage & 5.8E-5 & 1.0E-3 & 7.3E-4 & 5.2E-4 & 9.0E-7 & 9.1E-4 & 2.9E-4 \\
%Experiment shield & 1.5E-5 & 2.8E-4 & 1.9E-4 & 1.4E-4 & 0.0E+0 & 2.3E-4 & 8.1E-5 \\
%Mixing Chamber Stage & 4.5E-6 & 1.4E-4 & 1.1E-4 & 7.5E-5 & 0.0E+0 & 1.3E-4 & 4.1E-5 \\
%Cold Plate Stage & 1.1E-6 & 2.3E-5 & 1.7E-5 & 1.3E-5 & 2.1E-8 & 2.2E-5 & 6.9E-6 \\
%Still Stage & 5.4E-7 & 9.0E-6 & 7.4E-6 & 5.4E-6 & 0.0E+0 & 9.7E-6 & 2.7E-6 \\
%4K Stage & 1.7E-7 & 2.3E-6 & 1.5E-6 & 1.4E-6 & 0.0E+0 & 2.6E-6 & 4.8E-7 \\
%50K Stage & 1.9E-8 & 7.3E-7 & 4.7E-7 & 4.4E-7 & 6.3E-9 & 8.3E-7 & 2.0E-7 \\
%Vacuum Flange & 1.9E-8 & 3.4E-7 & 2.4E-7 & 2.3E-7 & 0.0E+0 & 3.8E-7 & 8.2E-8 \\
%Still Can & 3.6E-6 & 8.4E-5 & 6.9E-5 & 3.9E-5 & 0.0E+0 & 6.7E-5 & 3.3E-5 \\
%4K Can & 2.3E-6 & 3.9E-5 & 3.0E-5 & 2.1E-5 & 0.0E+0 & 3.6E-5 & 1.1E-5 \\
%Lower 50K Can & 1.9E-6 & 3.1E-5 & 2.4E-5 & 1.7E-5 & 2.1E-8 & 2.9E-5 & 9.2E-6 \\
%Upper 50K Can & 4.2E-8 & 1.4E-6 & 8.4E-7 & 8.1E-7 & 0.0E+0 & 1.5E-6 & 4.4E-7 \\
%Lower Vacuum Can & 1.6E-6 & 2.3E-5 & 1.7E-5 & 1.2E-5 & 0.0E+0 & 2.1E-5 & 7.7E-6 \\
%Upper Vacuum Can & 9.4E-8 & 9.9E-7 & 6.4E-7 & 5.7E-7 & 0.0E+0 & 1.1E-6 & 2.2E-7 \\
%\hline
    Source location & \iso{U}{238} & \iso{Th}{232} & \iso{K}{40} & Activation & \iso{Co}{60} & \iso{Cs}{137} & \iso{Pb}{210} \\
    \midrule
Interposer board & 7.1E+0 & 5.1E+0 & 1.5E+0 & 4.2E-1 & 3.1E-1 & 8.2E-1 & 1.5E+0 \\
%Packge Inner Surface & 2.0E +1 & 1.8E +1 & 9.8E-1 & 9.5E-1 & 7.8E-1 & 1.1E+0 & 3.8E+0 \\
Package & 7.3E-2 & 5.9E-2 & 1.3E-2 & 1.4E-2 & 2.1E-2 & 9.5E-3 & 6.8E-3 \\
%Package Outer Surface & 6.0E-3 & 6.4E-3 & 1.1E-3 & 6.8E-3 & 1.1E-2 & 3.6E-3 & 9.0E-5 \\
Experiment stage & 7.3E-4 & 1.0E-3 & 5.8E-5 & 5.2E-4 & 9.1E-4 & 2.9E-4 & 9.0E-7 \\
Experiment shield & 1.9E-4 & 2.8E-4 & 1.5E-5 & 1.4E-4 & 2.3E-4 & 8.1E-5 & 0.0E+0 \\
Mixing chamber stage & 1.1E-4 & 1.4E-4 & 4.5E-6 & 7.5E-5 & 1.3E-4 & 4.1E-5 & 0.0E+0 \\
Cold plate stage & 1.7E-5 & 2.3E-5 & 1.1E-6 & 1.3E-5 & 2.2E-5 & 6.9E-6 & 2.1E-8 \\
Still stage & 7.4E-6 & 9.0E-6 & 5.4E-7 & 5.4E-6 & 9.7E-6 & 2.7E-6 & 0.0E+0 \\
4K stage & 1.5E-6 & 2.3E-6 & 1.7E-7 & 1.4E-6 & 2.6E-6 & 4.8E-7 & 0.0E+0 \\
50K stage & 4.7E-7 & 7.3E-7 & 1.9E-8 & 4.4E-7 & 8.3E-7 & 2.0E-7 & 6.3E-9 \\
Vacuum flange & 2.4E-7 & 3.4E-7 & 1.9E-8 & 2.3E-7 & 3.8E-7 & 8.2E-8 & 0.0E+0 \\
Still can & 6.9E-5 & 8.4E-5 & 3.6E-6 & 3.9E-5 & 6.7E-5 & 3.3E-5 & 0.0E+0 \\
4K can & 3.0E-5 & 3.9E-5 & 2.3E-6 & 2.1E-5 & 3.6E-5 & 1.1E-5 & 0.0E+0 \\
Lower 50K can & 2.4E-5 & 3.1E-5 & 1.9E-6 & 1.7E-5 & 2.9E-5 & 9.2E-6 & 2.1E-8 \\
Upper 50K can & 8.4E-7 & 1.4E-6 & 4.2E-8 & 8.1E-7 & 1.5E-6 & 4.4E-7 & 0.0E+0 \\
Lower vacuum can & 1.7E-5 & 2.3E-5 & 1.6E-6 & 1.2E-5 & 2.1E-5 & 7.7E-6 & 0.0E+0 \\
Upper vacuum can & 6.4E-7 & 9.9E-7 & 9.4E-8 & 5.7E-7 & 1.1E-6 & 2.2E-7 & 0.0E+0 \\
    \bottomrule
    \end{tabular}
\end{table}

==> todo.tex <==
\section{To DO}
\begin{itemize}
    \item Figure 5 bar chart legend seems wrong (rate >1 MeV sometimes higher than total rate).
    \item{pretty up Figure 7}
    \item update table 9 (hit efficiencies)
    \item acknowledgements and author list
\end{itemize}
